Calibration to American Options: Numerical Investigation of the de-Americanization

American options are the reference instruments for the model calibration of a large and important class of single stocks. For this task, a fast and accurate pricing algorithm is indispensable. The literature mainly discusses pricing methods for American options that are based on Monte Carlo, tree and partial differential equation methods. We present an alternative approach that has become popular under the name de-Americanization in the financial industry. The method is easy to implement and enjoys fast run-times. Since it is based on ad hoc simplifications, however, theoretical results guaranteeing reliability are not available. To quantify the resulting methodological risk, we empirically test the performance of the de-Americanization method for calibration. We classify the scenarios in which de-Americanization performs very well. However, we also identify the cases where de-Americanization oversimplifies and can result in large errors.

==> tex/AccuracyStudy.tex <==
\subsection{Accuracy Study}
In this section we investigate the accuracy of our FEM solvers for the previously presented models for European options. Therefore, we define a test scenario of put and call options and illustrate the errors compared to benchmark solutions. More specifically, we only investigate here out-of-the-money options because later in the calibration methodology only out-of-the-money options are considered. \todo{oom options too short?} In our test setting we set $S_0=1$, $r=0.07$, $T=\{0.5,0.875, 1.25, 1.625,2\}$, for calls we set $K_{call}$ to ten equally distributed values in $[1,1.5]$ and for puts we set $K_{put}$ to ten equally distributed values in $[0.5,1]$. For the space and time discretization in our FEM solvers we set $\Delta t \approx 0.008$ and $\Delta h\approx 0.05$.


Figure \ref{Accuracy_CEV} illustrates the accuracy results for the CEV model. Here, we choose model parameters $\sigma=0.15$ and $\rho=0.75$ and as benchmark solution we implemented the closed-form solution of the CEV model for European put and call prices as shown in \cite{schroeder}. Overall, we observe that the absolute errors are in the $10^{-4}$ region. Naturally, we observe that at-the-money occur the highest option prices and the prices decrease in the out-of-money directions. By comparing put and call prices we see, that the call prices are higher than the put prices which can be explained by the local on the underlying value depending volatility. Furthermore we observe that the absolute error between benchmark and FEM solutions increases slightly with increasing maturities and that for put options the error is the highest in the close to at-the-money region, whereas for call options the error by going further out-of-the-money first increases, peaks at $K=1.2$ to $K=1.3$ and then decreases again.
\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/CEV_cloudpic.png} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/CEV_Diffs.png} 
  \end{minipage} 
  \caption{Accuracy study for the CEV model. Option prices (top) and absolute differences between benchmark and FEM solution (bottom)}
  \label{Accuracy_CEV} 
\end{figure} 

For the Heston model we used the closed-form solution in xx\todo{Olena: Add Source} as benchmark. Due to the fact, that this closed-form solution is only given for call option and put options would be derived via the put-call parity, we only focus on the out-of-the-money call options. As model parameters we use xx\todo{Olena: add parameters}. The accuracy results are summarized in Figure \ref{Accuracy_Heston}\todo{Discussion: Make Figure similar to other ones?}. Similar to the CEV model we observe absolut errors in the $10^{-4}$ region. As a slight difference to CEV model, here the highest error depend on the maturity
as well as the out-of-the-moneyness. In the at-the-money region we observe for a medium maturity $T=0.875$ the highest error, whereas deep out-of-the-money the highest maturity $T=2$ has the highest error. Additionally, for short ($T=0.5$) and high ($T=2$) maturities we observe that the error first increases and then similar to the CEV model decreases by going further out-of-the-money. For the other maturities the error just decreases by going further out-of-the-money.
\begin{figure} 
  \begin{minipage}{0.8\textwidth} 
     \centering 
     \includegraphics[width=0.8\textwidth]{./fig/03Sep15_market1_semianalytic_winkl10_dt008_DOF18721_2.png} 
 \end{minipage} 
  \caption{Accuracy study for the Heston model. Option prices (top) and absolute differences between benchmark and FEM solution (bottom)}
  \label{Accuracy_Heston} 
\end{figure} 

Lastly, Figure \ref{Accuracy_Merton} \todo{Remove title of Figure?} shows the results for the Merton model. Here, Fourier pricing is used as benchmark (xx) \todo{Max: Add source} and we select the following model parameters xx\todo{Max: Add parameters}. Similar to the previous models the error is in the $10^{-4}$ region. In contrast, we observe that the error decreases with increasing maturities except in the deep out-of-the-money regions.

\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Merton_cloudpic.png} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Merton_absDiffs.png} 
  \end{minipage} 
  \caption{Accuracy study for the Merton model. Option prices (top) and absolute differences between benchmark and FEM solution (bottom)}
  \label{Accuracy_Merton} 
\end{figure} 

Summarizing the accuracy study, we observe that for all models the absolute error between benchmark and FEM solution is in the $10^{-4}$ region and thus, we assume in the further studies of this paper, that our FEM solutions indeed represent the true price.\todo{Here I'm not sure with the formulation}

%\begin{figure} 
%  \begin{minipage}{0.8\textwidth} 
%     \centering 
%     \includegraphics[width=0.8\textwidth]{./fig/CEV_cloudpic.png} 
% \end{minipage} 
%  \begin{minipage}{0.8\textwidth} 
%     \centering 
%     \includegraphics[width=0.8\textwidth]{./fig/CEV_Diffs.png}} 
%  \end{minipage} 
%  \caption{Accuracy study for the CEV model. Option prices (top) and absolute differences between benchmark and FEM solution (bottom)}
%  \label{Accuracy_CEV} 
%\end{figure} 
%\begin{figure} 
%  \begin{minipage}{0.8\textwidth} 
%     \centering 
%     \includegraphics[width=0.8\textwidth]{./fig/Merton_cloudpic.png} 
% \end{minipage} 
%  \begin{minipage}{0.8\textwidth} 
%     \centering 
%     \includegraphics[width=0.8\textwidth]{./fig/Merton_absDiffs.png}} 
%  \end{minipage} 
%  \caption{Accuracy study for the Merton model. Option prices (top) and absolute differences between benchmark and FEM solution (bottom)}
%  \label{Accuracy_Merton} 
%\end{figure} 

==> tex/Models.tex <==
\section{Pricing Methodology}

In this section we will present a model formulation and numerical implementation
of the three investigated models (CEV, Heston, Merton). To
investigate the De--Ameri\-cani\-za\-tion methodology, we need to price American
and European options. \new{In general}, for European options there exists a
variety of fast pricing methodologies like e.g. Fast Fourier Transform
(\cite{schoutens}) or even closed-form solutions. For American options there
often do not exist closed-form solutions due to the early exercise possibility.
\new{Thus, one has to consider an appropriate numerical approximation for
American options. The common approaches for pricing P(I)DEs are the finite
differences method (FDM) and the finite elements method (FEM).
Here we restrict our consideration for the last one. For comparability purposes,
we
approximate European options also by FEM. We reformulate a problem in a weak
form, which leads to solve the corresponding variational equality
or inequality problem associated the European or American options respectively.
To solve the corresponding discrete variational inequalities, one can employ
one of the iterative methods like, e.g, Projected SOR
Algorithm,~\cite{achdou}, \cite{seydel} and Primal Dual Active Set
Strategy,~\cite{kunisch}. Here we present a methodology}
%Thus, driven by the the early exercise possibility of American options, we take
%the finite element method as solver. The finite element method allows to apply
%the PSOR algorithm (\cite{seydel}) or the primal dual approach
%(\todo{reference}) to solve variational inequalities resulting from this early
%exercise possibility. European options are also
%priced with the finite elements. 

Our market data in the numerical study later on will be Google market data. As Google does not pay dividends, we can neglect dividend payments in our pricing methodology. Following \cite{binghamkiesel}, we treat American calls accordingly as European calls whenever possible.
%--------------------------------------------------------------------------------------------------------------------------------------------
%                CEV model
%--------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Option Pricing Models}
We provide a brief introduction to the models we use for our study, namely the
constant elasticity of variance model (CEV), the stochastic volatility Heston
model, and the Merton model.

Consider an asset price dynamics $S_\tau$ governed by the following stochastic
differential equation (SDE)
\begin{subequations}\label{SDE1}
\begin{equation}
\d{S_\tau}=\ rS_\tau\d{\tau} + \sigma(S,\tau) S_\tau \d{W_\tau}+
S_{\tau-}\d{J_\tau},\qquad S_0=s\ge0,
\end{equation}
\begin{equation}
J_\tau =\ \sum_{i=0}^{N_\tau} Y_i,
\end{equation}
\end{subequations}
%\begin{align}
%\d{S_\tau}=&\ rS_\tau\d{\tau} + \sigma(S,\tau) S_\tau \d{W_\tau}+
%S_{\tau-}\d{J_\tau},\qquad S_0=s\ge0,\\
%J_\tau =&\ \sum_{i=0}^{N_\tau} Y_i,
%\label{SDE1}
%\end{align}
with the Wiener process $dW_\tau$, interest rate $r$ and a volatility
$\sigma(S,\tau)$.
The jump part $(J_\tau)_{\tau\geq 0}$ is governed by a compound Poisson process
with intensity $\lambda\geq 0$ and independent identically distributed jumps
$Y_i$, $i\in\IN$, that are independent from the Poisson process
$(N_\tau)_{\tau\geq 0}$.

For the standard Black-Scholes model, we pose an assumption on
the volatility
$\sigma(S,\tau)=\sigma=const$, set the jump intensity $\lambda=0$ and obtain that the process~\eqref{SDE1} is a
standard Brownian motion. It turns out, that this assumption is often violated
by the market. Several models were developed to
extend a Black-Scholes model to a model with a non-constant volatility, e.g.,
CEV and Heston models.\\

As local volatility model we present the CEV model, introduced by \cite{Cox}. Here the local volatility is assumed to be a deterministic function of the asset price for the process in~\eqref{SDE1}
$\sigma(S,\tau)=\sigma S_\tau^{\zeta-1}$, $0<\zeta<1$ (jump intensity $\lambda=0$).\\

As stochastic volatility model we use the Heston model, \cite{heston}. In contrast to the CEV model, the Heston model considers volatility as a stochastic variable, and the model is based on the dynamics of the both: the stock price~\eqref{SDE1}, with jump intensity $\lambda=0$, and the
volatility $v_\tau$~\eqref{SDE2},
\begin{equation}
 dv_\tau=\kappa(\gamma-v_\tau)dt + \xi\sqrt{v_\tau}d\widetilde{W}_\tau,
 \label{SDE2}
\end{equation}
with $v_\tau=\sigma^2$, a mean variance $\gamma>0$, a rate of mean reversion
$\kappa>0$ and a volatility of volatility $\xi>0$. The Wiener processes
$W_\tau$
and $\widetilde{W}_\tau$ are correlated with the correlation parameter
$\rho\in
[-1,1]$. The
process~\eqref{SDE2} is also referred as a CIR (Cox-Ingersoll-Ross) process. In both, the CEV and Heston model, jumps aren't included.\\

Another class of models are jump-diffusion models. The Merton model extends the Black-Scholes model by adding jumps. The log-asset price process is not driven by a Brownian motion exclusively, but by a jump-diffusion process, instead. Thus, in the Merton model of \cite{Merton1976}, the volatility of the asset process is still assumed to be constant, 
	\begin{equation}
		\sigma(S,\tau) \equiv \sigma>0,\qquad \forall S>0, \forall
\tau\geq 0.
	\end{equation}
but being a jump diffusion model, the jump intensity $\lambda>0$ is positive and $N_t\sim \text{Poiss}(\lambda t)$. Jumps are taken to be independent normally distributed random variables,
	\begin{equation}
		Y_i \sim \mathcal{N}(\alpha,\beta^2)
	\end{equation}	 
with expected jump size $\alpha\in\IR$ and standard deviation $\beta>0$. A trajectory of the Merton model illustrating the jump feature is displayed in Figure~\ref{fig:deAmMertonSingleTrajectory}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig.: BS Model trajectories
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\makebox[0pt]{\includegraphics[scale=0.7]{fig/max/MertonTrajectory/deAmMertonSingleTrajectory}}
\caption{An asset price trajectory in the Merton model with $S_0=1$ and $r=0.03$. Note the existence of jumps in the trajectory.}
\label{fig:deAmMertonSingleTrajectory}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Pricing P(I)DE}

With the use of It\^o formula, we can reformulate all models in
terms of the partial (integro-) differential equation (P(I)DE).
Denote by
$t=T-\tau$ a time to
maturity $T$, $T<\infty$, by $K$ a strike of an option. We work with the
log-transformed
stock variable $x:=\log\left(\frac{S}{K}\right)$ for the Heston and Merton
models, for the CEV model we stay in the S variable, $S\in(0,\infty)$, $x\in(-\infty,\infty)$. %This is a standard practice in option pricing modeling, which allows to eliminate variable coefficients. 
Denote the price of an option
$P:(0,T)\times\mathbb{R}^n\rightarrow\mathbb{R}^+$ ($n=1,2$). The value of an
option at $t=0$ is given by the pay-off function
$\widetilde{\mathcal{H}}(\cdot)$,
$P(0)=P_0=\widetilde{\mathcal{H}}$ with $\widetilde{\mathcal{H}}(x):=(Ke^x-K)_+$
($\widetilde{\mathcal{H}}(x):=(K-Ke^x)_+$) for a call (put) in the Heston and
Merton model.
In the CEV model we have $\widetilde{\mathcal{H}}(S):=(S-K)_+$ or
$\widetilde{\mathcal{H}}(S):=(K-S)_+$
for a call or put respectively.

Then to find a value of the European option $P$, paying
$P_0=\widetilde{\mathcal{H}}(x)$ ($P_0=\tilde{\mathcal{H}}(S)$) at
$t=0$,
leads to solve the following initial boundary value problem
\begin{align}
\frac{\partial P}{\partial t}-\mathcal{L}P=0,\quad P(0)=P_0,
\label{EO_PDE}
\end{align}
where the spatial partial (integro-) differential operator
$\mathcal{L}:=\mathcal{L}^s$, $s=\{\rm CEV, H, M\}$ is
determined by the model used to price an option. 
For the CEV, Heston and Merton it is given
in~\eqref{L_CEV},~\eqref{L_Heston} and~\eqref{L_Merton}
respectively.
\begin{subequations}
 \begin{align}
 \mathcal{L}P^{\rm CEV}:&=\frac{\sigma S_\tau^{\zeta-1}}{2}S^2\frac{\partial^2 P}{\partial S^2}+rS\frac{\partial P}{\partial S}-rP \label{L_CEV},\\
\mathcal{L}P^{\rm H}:&=\frac{1}{2}v\frac{\partial^2 P}{\partial
x^2}+\xi v\rho\frac{\partial^2
P}{\partial v\partial x}+\frac{1}{2}\xi^2v\frac{\partial^2 P}{\partial
v^2}+\kappa(\gamma-v)\frac{\partial P}{\partial
v}+\left(r-\frac{1}{2}v\right)\frac{\partial P}{\partial
x}-rP,\label{L_Heston}\\
\mathcal{L}P^{\rm M}:&= b\partial_x P(x) + \frac{1}{2}\sigma^2\partial_{xx}P(x)
+ \int_\IR (P(x+z)-P(x)-\partial_x P(x)z)F(\d{z})-rP \label{L_Merton},
\end{align}\label{model_operators}
\end{subequations}
wherein for the Merton model the jump measure $F$ is
given by
	\begin{equation}
		F(\d{z}) = \frac{\lambda}{\sqrt{2\pi\beta^2}}\exp\left(-\frac{(z-\alpha)^2}{2\beta^2}\right)\d{z}
	\end{equation}
and the drift $b\in\IR$ is set to $b:=r -
\frac{1}{2}\sigma^2-\lambda\left(e^{\alpha+\frac{\beta^2}{2}}-1\right)$ due to
the no-arbitrage condition. 


Pricing an American option (e.g., put), due to its early exercise possibility,
results in
additional inequality constraints, and leads to solve the following system of
inequalities
\begin{subequations}
 \begin{align}
\frac{\partial P}{\partial t}-\mathcal{L}P\geq 0, \quad  P-P_0&\geq 0,\\
\left(\frac{\partial P}{\partial
t}-\mathcal{L}P\right)\cdot\left(P-P_0\right)&=0.
\end{align}
\label{AO_put_model}
\end{subequations}


We denote a parameter vector
$\parmu:=(\xi,\rho,\gamma,\kappa,r)\in\mathbb{R}^5$ for the Heston model,
$\parmu:=(\sigma, \zeta)\in\mathbb{R}^2$ for the CEV and $\parmu:=(\sigma,
\alpha, \beta, \lambda)\in\IR^4$ for the Merton model. 
\new{Then the
problems~\eqref{EO_PDE},~\eqref{AO_put_model} are parametrized problems w.r.t.
$\parmu\in\mathcal{P}$, where $\mathcal{P}\subset\mathbb{R}^n$ is a parameter
space. The solution can be written as $P=P(\parmu)$. In some case, for notational convenience, we will omit the parameter dependence of $P$ and related quantities.}

%-------------------------------------------------------------------------------
%               Var Form
%-------------------------------------------------------------------------------
\subsection{Variational Formulation}
As a next step we pose the problem in the weak from ans introduce the variational formulation for all 3 models.
\subsubsection{CEV and Heston model}
\new{For the CEV and Heston model we localize the
problems to an open bounded domain
$\Omega\subset\mathbb{R}^n$, $n=1,2$. It is defined as
$\Omega:=(S_{\min},S_{\max})\subset\mathbb{R}^1$ for the CEV model and as
$\Omega:=(v_{\min},v_{\max})\times(x_{\min},x_{\max})\subset\mathbb{R}^2$,
$v_{\min}>0$ for the Heston model.
The functional spaces for the CEV and Heston models are introduced
in~\eqref{V_CEV},~\eqref{V_Heston} respectively.}
\begin{align}
V:&=\{v\in L^2(\Omega):S\frac{\partial v}{\partial S}\in L^2(\Omega)\},\label{V_CEV}\\
 V:&=\{\phi\in H^1(\Omega):\quad \phi=0\quad\text{on }\partial\Omega_D\}, \label{V_Heston}
\end{align}
where $\partial\Omega_D$ denotes a Dirichlet
portion of the boundary $\partial\Omega$. Define $V^{\prime}$ to be the dual
space of $V$ and denote by $\langle\cdot,\cdot\rangle$ a duality pairing between
$V$ and $V^{\prime}$ and by $(\cdot,\cdot)$ an inner product on $L^2(\Omega)$.
Denote a temporal interval $I:=[0,T]$, $T>0$.

Introduce bilinear forms $a^s: V\times V\rightarrow\mathbb{R}$, $s=\{\rm
CEV, H\}$ for the CEV and the Heston models,
\begin{subequations}
 \begin{align}
a^{\rm CEV}(\psi,\phi;\parmu)&:=\int_{\Omega} \frac{\sigma
S^{2\zeta}}{2}\frac{\partial \psi}{\partial S}\frac{\partial \phi}{\partial S}dS
+ r\int_{\Omega} \psi\phi dS
+\int_{\Omega}(-rS+\zeta\sigma^2S^{2\zeta-1})\frac{\partial\psi}{\partial S}\phi
dS,\\
a^{\rm H}(\psi,\phi;\parmu)&:=\int_{\Omega}A\nabla \psi\nabla\phi+\int_{\Omega}
b\cdot\nabla
\psi\phi+r\int_{\Omega}\psi\phi\label{bil_heston}
 \end{align}
 \label{bil_form}
\end{subequations}
wherein for the Heston model in~\eqref{bil_heston}, $\nabla
:=\left(\frac{\partial}{\partial v},\frac{\partial}{\partial x}
\right)^T$, $A$ and $b$ as in~\eqref{heston_coef}, i.e, 
\begin{eqnarray}
A:=\frac{1}{2}v\begin{bmatrix}
\xi^2 &\rho\xi \\ \rho\xi &1
\end{bmatrix}, \ \ \ \ \ \ \ \ \ \ \ \ 
b:=\begin{bmatrix}
-\kappa(\gamma-v)+\frac{1}{2}\xi^2 \\ -r+\frac{1}{2}v+\frac{1}{2}\xi\rho
\end{bmatrix}.\label{heston_coef}
\end{eqnarray}

Then a weak from of~\eqref{EO_PDE} for the CEV and
Heston models reads as follows,~\cite{achdou},: Find $u(\parmu)\in
L^2(I;V)\cap C^0(I;L^2(\Omega))$ with $\frac{\partial
u(\parmu)}{\partial t}\in L^2(I;V')$, $f(\parmu)\in L^2(I;V^{\prime})$, $u_0(\parmu)\in L^2(\Omega)$,
such that for a.e. $t\in I$ holds
\begin{subequations}
 \begin{align}
\left\langle\frac{\partial u}{\partial
t}(t;\parmu),\phi\right\rangle+a(u(t;\parmu),\phi;\parmu)&=\langle f(t;\parmu),\phi\rangle,
\quad\phi\in V,\label{eq:weak1}\\
u(0;\parmu)&=u_0(\parmu),\label{eq:weak2}
\end{align}
\label{EO_weak}
\end{subequations}
where 
\begin{equation}
 \langle f(t;\parmu),\phi\rangle=-a(u_L(t;\parmu),\phi)-\left\langle\frac{\partial
u_L}{\partial
t}(t;\parmu),\phi\right\rangle.
\end{equation}
\new{and $u(0;\parmu)=P(0;\parmu)-u_L(0;\parmu)$, the modified payoff is
$\mathcal{H}(t;\parmu):=\widetilde{\mathcal{H}}-u_L(t;\parmu)$}. Here $u_L(\parmu)$ is a Dirichlet
lift function, $u_L(\parmu)\in
L^2(I;V)\cap C^0(I;L^2(\Omega))$ with $\frac{\partial
u_L}{\partial t}(\parmu)\in L^2(I;V')$, such that $u_L(t;\parmu)=g(t;\parmu)$ on
$\partial\Omega_D$, where the function of the boundary values $g$ is 
defined
in Section~\ref{sec_bc}. Then the price of an option in~\eqref{EO_PDE} is given
as $P=u(\parmu)+u_L(\parmu)$.

\new{With the use of the above notations, we present the variational
formulation for American options.}
Introduce a closed convex subset
$\mathcal{K}(t;\parmu)\subset V$, 
\begin{equation}
 \mathcal{K}(t;\parmu):=\{\phi\in V:\quad \phi\geq\new{\mathcal{H}(t;\parmu)}, \quad\text{in 
}\Omega\},
\end{equation}
where the inequality is understood in a pointwise sense. Then the weak form
of~\eqref{AO_put_model},~\cite{achdou}, reads as follows: \new{Given
$u_0(\parmu)\in\mathcal{K}(\parmu)$, find $u(\parmu)\in
L^2(I;V)\cap C^0(I;L^2(\Omega))$
with $\frac{\partial
u}{\partial t}(\parmu)\in L^2(I;V')$, such that $u(t;\parmu)\in\mathcal{K}(t;\parmu)$ for a.e. $t\in I$
and the following holds for all $\phi\in\mathcal{K}(t;\parmu)$ }
\begin{subequations}
 \begin{align}
\left\langle\frac{\partial u}{\partial
t}(t;\parmu),\phi-u(t;\parmu)\right\rangle+a(u(t;\parmu),\phi-u(t;\parmu);\parmu)&\geq
\left\langle f(t;\parmu),\phi-u(t;\parmu)\right\rangle,\\
u(0;\parmu)&=u_0(\parmu),
\end{align}\label{AO_weak}\end{subequations}
where \new{$u(0;\parmu)=P(0;\parmu)-u_L(0;\parmu)$} and the price of an American put
option~\eqref{AO_put_model} is determined as
$P(\parmu)=u(\parmu)+u_L(\parmu)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Merton model}\todo{add description of $\Omega$ and parameter dependency}
For the Merton model a weak solution $u$ exists in the solution space, $u\in
L^2(I;V)\cap C^0(I;H)$ with $\frac{\partial u}{\partial t}\in L^2(I;V')$, where 
	\begin{equation}
		V = H_\eta^1(\IR),\quad H = L^2(\IR),
	\end{equation}
wherein $H_\eta^1(\IR)$ denotes the appropriately weighted Sobolev-Slobodeckii space, see \cite{EberleinGlau2012} for further details. Before we can apply Finite Element solvers to derive the Merton price some modifications of the PIDE are performed. We subtract a function $\Psi$ from the original pricing PIDE that approximately matches the behavior of $P^\text{Merton}$ such that for all $t\in[0,T]$ we have $\widetilde{P}^\text{Merton} = P^\text{Merton}(t,x)-\Psi(t,x)\rightarrow 0$ for $x\rightarrow\pm \infty$.
We choose
	\begin{equation}
	\label{eq:MertonPsi}
		\begin{split}
			\Psi^\text{Am./Eu. call}(t,x) =&\ (Ke^x - Ke^{-rt})\Phi(x),\\
			\Psi^\text{Am. put}(t,x) =&\ (K-Ke^x)(1-\Phi(x)),
		\end{split}
	\end{equation}
for European call and put options, respectively, wherein $\Phi$ is the
cumulative distribution function of the Normal distribution~\eqref{cum_nd},
\begin{equation}
 \Phi(x)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^x
e^{-\frac{1}{2}z^2}dz.
\label{cum_nd}
\end{equation}



The solution $u$ to the resulting PIDE thus decays to zero for $x\rightarrow \pm\infty$. We choose $x_\text{min}<x_\text{max}$ with $|x_\text{min}|$, $|x_\text{max}|$ large enough and truncate the infinite domain $\IR$ to $[x_\text{min},x_\text{max}]$ assuming zero boundary conditions,
	$$
			\widetilde{P}^\text{Merton}(x)=\ 0,\qquad\text{for    }
x\leq x_\text{min},\quad\quad
			\widetilde{P}^\text{Merton}(x)=\ 0,\qquad\text{for    }
x\geq x_\text{max}.
$$
The associated bilinear form is then given as
\begin{equation}
	\begin{split}
		a^\text{Merton}(\varphi,\psi) =&\ -b\int_\IR(\partial_x\varphi(x))\psi(x)\d{x}+\frac{1}{2}\sigma^2 \int_\IR\partial_{x}\varphi(x)\partial_x\psi(x)\d{x}\\
		&\quad -\int_\IR\int_\IR(\varphi(x+y)-\varphi(x))F(\d{y})\psi(x)\d{x} +r\int_\IR\varphi(x)\psi(x)\d{x}
	\end{split}\end{equation}
for all $\varphi,\psi\in H_0^1(\IR)$ from which the weak formulation arises which is given by 
	\begin{subequations}
	\begin{align}
		\left\langle\frac{\partial u}{\partial t}(t),\phi\right\rangle+a^\text{Merton}(u(t),\phi)&=\langle f(t),\phi\rangle, \quad\forall\phi\in V,\label{eq:Mertonweak1}\\
		u(0)&=u_0,\label{eq:Mertonweak2}
	\end{align}
	\label{eq:Mertonweak}
	\end{subequations}
where $u_0(x)=\new{\widetilde{\mathcal{H}}(x)} - \Psi(0,x)$ and
	\begin{equation}
		\langle f(t),\phi\rangle= -\left\langle \frac{\partial}{\partial t}\Psi(t),\phi\right\rangle- a^\text{Merton}(u(t),\phi),\quad \forall \phi\in V.
	\end{equation}
%
%
%	\begin{equation}
%	\begin{split}
%		a(\cdot,\cdot) =&\ a^\text{Merton}(\cdot,\cdot),\\
%		f =&\  -\frac{\partial}{\partial t} \Psi - a^\text{Merton}(\Psi,\cdot),\\
%		u_0 =&\ \mathcal{H} - \Psi.
%	\end{split}
%	\end{equation}
Having solved the associated scheme, the price of the option is derived by
setting $P^\text{Merton} = u+\Psi$.


%-------------------------------------------------------------------------------
%               Boundary conditions
%-------------------------------------------------------------------------------
\subsubsection{Discretization}

We discretize the problem~\eqref{EO_weak},~\eqref{AO_weak}
and \eqref{eq:Mertonweak}, respectively, in time with $\theta$-scheme ($\theta=1$ for an implicit Euler and $\theta=\frac{1}{2}$ for the Crank-Nikolson scheme) and in space with a standard
conforming piecewise linear finite elements. 

We divide the interval $[0,T]$ into
$L$ subintervals of equal length $\Delta
t:=\frac{T}{L}$ and $t^k:=k\Delta t$, $0<k\leq L$. We denote $V_{h}\subset V$,
$h>0$, to be a finite-dimensional subspace of  $V$ with $\dim
V_{h}=\mathcal{N}<\infty$. Consider a triangulation $\mathcal{T}_\mathcal{N}$ of
$\Omega$, consisting of
$J$ simplices $T_\mathcal{N}^j$, $1\leq j\leq J$, such
that
$\overline{\Omega}=\cup_{T_\mathcal{N}\in\mathcal{T}_\mathcal{N}}\overline{T}
_\mathcal{N}$. We define the discrete space 
\begin{equation}
 V_h:= \{v \in V:\quad v_{|T_\mathcal{N}^j}\in\mathbb{P}^1(T_\mathcal{N}^j),
\quad 1\leq j\leq J \}.
\end{equation}
The basis functions $\phi_i \in V_h$ are associated with its Lagrange 
node $m_i\in\overline{\Omega}$, i.e., $\phi_i(m_j) =\delta_{ij}$, for
$i,j=1,\ldots,\mathcal{N}$. \new{Then the solution $u(t;\parmu)\in V$ is approximated
by $u_h^k(\parmu)\in V_h$, $0<k\leq L$}. For \new{notational convenience, we omit a
subscript $h$ in
$V_h$ and all associated quantities, and consider them as a
discrete ones.}

The discrete problem of~\eqref{EO_weak} reads as follows:
Given $u^0(\parmu)\in V$, find $u^{k+1}(\parmu)\in V$,  for $0<k\leq L-1$, such that for
all
$\phi\in V$ holds
 \begin{align} 
 \frac{1}{\Delta
t}(u^{k+1}(\parmu)-u^k(\parmu),\phi)+a(\theta u^{k+1}(\parmu)+(1-\theta)u^k(\parmu),\phi;\parmu)&=f^{k+1}(\phi;\parmu).\label{pr_det}
 \end{align}

 
 
\new{For the numerical treatment of the variational inequality~\eqref{AO_weak},
it
is convenient to rewrite it in a variational saddle point form, where the
constrains are imposed by the means of the Lagrange multiplier
$\lambda$,~\cite{kikuchi}. Let $W:=V^{\prime}$ and $M\subset W$ is a closed non
empty convex cone. Introduce a bilinear form $b:W\times
V\rightarrow\mathbb{R}$, defined as
$b(\eta,\phi)=\langle\eta,\phi\rangle$. For $0<k\leq L-1$ introduce a
functional $g^{k+1}(\parmu)\in W^{\prime}$, as
$g^{k+1}(\eta;\parmu)=b(\eta,\mathcal{H}^{k+1}(\parmu))=b(\eta,\widetilde{\mathcal{H}}-u_L^{k+1
}(\parmu) )$.} The
discrete problem of~\eqref{AO_weak} reads as follows: Given initial data
$u^0(\parmu)\in V$, find $(u^{k+1}(\parmu),\lambda^{k+1}(\parmu))\in V\times M$ for $0<k\leq L-1$,
such that for all
$\phi \in V,\eta \in M$ the following holds 
\begin{align}
&\frac{1}{\Delta
t}(u^{k+1}(\parmu)-u^k(\parmu),\phi)+a(\theta u^{k+1}(\parmu)+(1-\theta)u^k(\parmu),\phi;\parmu)
-b(\lambda^{k+1}(\parmu),\phi)  =  f^{k+1}(\phi;\parmu),\\
&b(\eta-\lambda^{k+1}(\parmu),u^{k+1}(\parmu))  \geq g^{k+1}(\eta-\lambda^{k+1}(\parmu);\parmu).
\end{align}


\subsubsection{Boundary Conditions}\label{sec_bc}
\new{As we have specified previously, we tackle the non-homogeneous truncated
Dirichlet boundary conditions, by means of the lift function $u_L(t)=g(t)$ on
$\partial{\Omega}_D$. For all models we consider only Dirichlet or Neumann types
of boundary conditions. For the European call in the Heston model, we specify
them similar to~\cite{winkler2001},}
\begin{subequations}
\begin{align}
\Gamma_1: \ &\vol=\vol_{\min}\ \ \ \
&&P(t,\vol_{\min},x)=Ke^{x}\Phi(d_1)-Ke^{-rt}\Phi(d_2),\\
\Gamma_2: \ &\vol=\vol_{\max}\ \ \ \ &&P(t,\vol_{\max},x)=Ke^{x},
\end{align}\label{bc_log_eo}\end{subequations}
and on the boundaries  $\Gamma_3=\{x=x_{\min}\}$ and $\Gamma_4=\{x=x_{\max}\}$, we interpolate linearly.
The cumulative
distribution function
$\Phi(\cdot)$ is defined in~\eqref{cum_nd} and $d_{1,2}=\frac{x+(r\pm\frac{\sigma^2}{2})t}{\sigma\sqrt{t}}$ with
$\sigma=\sqrt{\vol}$.

The boundary conditions for American put options in the Heston model are as
follows,~\cite{clarke, during},
\begin{align*}
 P(t,\vol,x)&=\widetilde{\mathcal{H}}(x), &&\text{on}\quad\Gamma_3\cup\Gamma_4,
&&&\\
 \frac{\partial P}{\partial \vol}(t,\vol_{\min},x)&=0,
&&\text{on}\quad\Gamma_1,
 &&&\frac{\partial P}{\partial \vol}(t,\vol_{\max},x)=0, \ \
\text{on}\quad\Gamma_2.
\end{align*}

For the CEV model, following \cite{seydel}, we applied the boundary conditions
\begin{align}
P(t,S_{min})&=0,\quad P(t,S_{max})=S_{max}-e^{-rt}K,\quad &\text{for call options},\\
P(t,S_{min})&=e^{-rt}K-S_{min},\quad P(t,S_{max})=0,\quad &\text{for European put options,}\\
P(t,S_{min})&=K-S_{min},\quad P(t,S_{max})=0,\quad &\text{for American put options}.
\end{align}

The transformation of the Merton model by subtraction of an appropriately chosen
function $\Psi$ as introduced in~\eqref{eq:MertonPsi} results in zero boundary
conditions in space, $u(t,x_\text{min}) = u(t,x_\text{max}) = 0$ for all $t\in
[0,T]$.

==> tex/Old/numerical_study.tex <==
\section{Numerical Study of De--Ameri\-cani\-za\-tion effects} 
Our main objective is to investigate the De--Ameri\-cani\-za\-tion methodology with respect to calibration. How accurate does this methodology work and if there are differences, how crucial are these. But before we look at calibration in detail, we present an accuracy study of our FEM pricers followed by an investigation of De--Ameri\-cani\-za\-tion effects on pricing. Then we switch to calibration to synthetic data and finally, market data.

\subsection{Accuracy Study}
Here we investigate the accuracy of our FEM solvers for the previously presented models for European options. Therefore, we define a test scenario of put and call options and illustrate the errors compared to benchmark solutions. %More specifically, we only investigate here out-of-the-money options because later in the calibration methodology only out-of-the-money options are considered. \todo{oom options too short?} 
In our test setting we set $S_0=1$, $r=0.07$, $T=\{0.5,0.875, 1.25, 1.625,2\}$ and we set $K$ to 21 equally distributed values in $[0.5,1.5]$. For the discretization we set $[S_min,S_max]=[0.01,2]$ for the CEV model, $[v_{min}, v_{max}]=[10^{-5},3]$ and  $[x_{min}, x_{max}]=[-5,5]$ for the Heston model and for the Merton model we set $[x_{min}, x_{max}]=[,]$. We set $\mathcal{N}=1000$ for the CEV model, $\mathcal{N}=49\times 97=4753$ for the Heston model and for the Merton model $\mathcal{N}=$, and $\Delta t = 0.008$ for all models.

Figure \ref{Accuracy_CEV_Puts} illustrates the accuracy results for put options in the CEV model. Here, we choose model parameters $\sigma=0.15$ and $\rho=0.75$ and as benchmark solution we implemented the closed-form solution of the CEV model for European put and call prices as shown in \cite{schroeder}. Overall, we observe that the absolute errors are in the $10^{-4}$ region. Naturally, we observe that in-the-money occur the highest option prices and the prices decrease in the out-of-money directions. Figure \ref{Accuracy_CEV_Puts} shows the results for call options. By comparing put and call prices we see, that the call prices are higher than the put prices which can be explained by the locally on the underlying value depending volatility. 
Furthermore we observe that the absolute error between benchmark and FEM solutions increases slightly with increasing maturities.
% and that for put options the error is the highest in the close to at-the-money region, whereas for call options the error by going further out-of-the-money first increases, peaks at $K=1.2$ to $K=1.3$ and then decreases again.
\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Puts_Price.jpg} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Puts_Diffs.jpg} 
  \end{minipage} 
  \caption{Accuracy study for put options in the CEV model. Option prices (left) and absolute differences between benchmark and FEM solution (right)}
  \label{Accuracy_CEV_Puts} 
\end{figure} 

\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Call_Prices.jpg} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Call_Diffs.jpg} 
  \end{minipage} 
  \caption{Accuracy study for call options in the CEV model. Option prices (left) and absolute differences between benchmark and FEM solution (right)}
  \label{Accuracy_CEV_Calls} 
\end{figure} 
%
%%  %%%%%%%%%%%%%%%%%% Heston model accuracy %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
For the Heston model we used the closed-form solution in~\citep{janek2011fx} as benchmark. As model parameters we use $\parmu=(0.1, -0.5, 0.05, 1.2, 0.001)$ with $v_0=0.05$. The accuracy results for put and call options using a closed-form solution are summarized in Figure~\ref{Accuracy_Heston_Semi_put} and Figure~\ref{Accuracy_Heston_Semi_call} respectively. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Heston (put)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h!]
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_put_winkl10_dt008_DOF18721_FourSOL}
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_put_winkl10_dt008_DOF18721_FourDIF} 
%     \caption{Accuracy study for put options in the Heston model. Left: Option prices obtained using the Fourier method (circles) and the FEM method (stars). Right: The respective absolute differences.}
%     \label{Heston_Fourier_put}
%   \end{figure}    

\begin{figure}[h!]    
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_put_stand10_dt008_DOF4753_SemiSOL.png}
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_put_stand10_dt008_DOF4753_SemiDIF.png} 
     \caption{Accuracy study for put options in the Heston model. Left: Option prices obtained with the semiclosed formula (circles) and the FEM method (stars). Right: The respective absolute differences.}
     \label{Accuracy_Heston_Semi_put}
   \end{figure}    


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Heston (call)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h!]
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_call_winkl10_dt008_DOF18721_FourSOL}
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_call_winkl10_dt008_DOF18721_FourDIF} 
%     \caption{Accuracy study for call options in the Heston model. Left: Option prices obtained using the Fourier method (circles) and the FEM method (stars). Right: The respective absolute differences.}
%      \label{Heston_Fourier_call}
%   \end{figure}    

\begin{figure}[h!]   
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_call_stand10_dt008_DOF4753_SemiSOL.png}
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_call_stand10_dt008_DOF4753_SemiDIF.png} 
     \caption{Accuracy study for call options in the Heston model. Left: Option prices obtained with the semiclosed formula (circles) and the FEM method (stars). Right: The respective absolute differences.} \label{Accuracy_Heston_Semi_call}
   \end{figure}    


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Lastly, Figure~\ref{fig:Accuracy_Merton_Puts} shows the results for European put options and Figure~\ref{fig:Accuracy_Merton_Calls} shows the results for European call options in the Merton model. Here, Fourier pricing is used as benchmark. For this accuracy study, the model is parametrized setting $\sigma=0.2$, $\alpha=-0.1$, $\beta=0.1$ and $\lambda=3$. In both figures, the interest rate $r$ has been chosen at a rather high rate, $r=7\%$. Similarly to the previous models the error is in the $10^{-4}$ region. In contrast, we observe that the error decreases with increasing maturities except in the deep out-of-the-money regions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Merton (put)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_putcloudpic} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_putAbsDiff} 
  \end{minipage} 
  \caption{Accuracy study for put options in the Merton model. Left: Option prices from the reference method (circles) and the FEM method (stars). Right: The respective absolute differences.}
  \label{fig:Accuracy_Merton_Puts} 
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Merton (call)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_callcloudpic} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_callAbsDiff} 
  \end{minipage} 
  \caption{Accuracy study for call options in the Merton model. Left: Option prices from the reference method (circles) and the FEM method (stars). Right: The respective absolute differences.}
  \label{fig:Accuracy_Merton_Calls} 
\end{figure} 

Summarizing the accuracy study, we observe that for all models the absolute error between benchmark and FEM solution is in the $10^{-3}$ to the $10^{-4}$ region.

\subsection{Effects of De--Ameri\-cani\-za\-tion on Pricing}
\label{sec:Pricing}

After we have presented our models, we want to firstly focus on differences caused by the De--Ameri\-cani\-za\-tion itself. Therefore, we compare de--americanized American prices with derived European option prices as illustrated in Figure \ref{DeAmPricing} and analyze the differences. 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/DeAmPricing.png}
\caption{First Step De--Ameri\-cani\-za\-tion: Focus on pricing differences}
\label{DeAmPricing}
\end{center}
\end{figure}

The advantage of this approach is that we can purely focus on the De--Ameri\-cani\-za\-tion without mixing it with any calibration issues. In order to do so, we defined the following test set for the range of investigated options. Here we focus on put options due to the fact that non dividend payments lead to the same prices for American and European calls.
\begin{align}
S_0&=1\notag\\
K&=0.80,0.85,0.90,0.95,1.00,1.05,1.10,1.15,1.20\notag\\
T&=\frac{1}{12},\frac{2}{12},\frac{3}{12},\frac{4}{12},\frac{6}{12},\frac{9}{12},\frac{12}{12},\frac{24}{12}\notag\\
r&=0, 0.01, 0.02, 0.05,0.07\label{DeAm_Pricing_Setting}
\end{align}
In each model, 5 parameter sets are investigated to cover the parameter range. These are summarized in Table \ref{Tab_Parameters_Pricing}. 
\begin{table}[h!]
\centering
\begin{tabular}{ccc|ccccc|cccc}
      & \multicolumn{2}{c|}{CEV} & \multicolumn{5}{c|}{Heston}                    & \multicolumn{4}{c}{Merton} \\
      & $\sigma$   & $\xi$ & $\zeta$ & $\rho$ & $\gamma$ & $\kappa$ & $v_0$ & $\sigma$ & $\alpha$    & $\beta$    & $\lambda$ \\ \hline
$p_1$ & $0.2$      & $0.5$ & 0.10     & -0.20      & 0.07     & 0.1      & 0.07  & 0.20      &  -0.01      & 0.01       & 1 \\
$p_2$ & $0.275$    & $0.6$ & 0.25     & -0.50   & 0.10     & 0.4      & 0.10  & 0.15     &  -0.05      & 0.05       & 2 \\
$p_3$ & $0.35$     & $0.7$ & 0.40     & -0.50    & 0.15     & 0.6      & 0.15  & 0.20      &  -0.10       & 0.10        & 3 \\
$p_4$ & $0.425$    & $0.8$ & 0.55     & -0.45   & 0.20     & 1.2      & 0.20  & 0.10      &  -0.10       & 0.20        & 5 \\
$p_5$ & $0.5$      & $0.9$ & 0.70     & -0.80    & 0.30      & 1.4      & 0.30  & 0.10      &  -0.15      & 0.20        & 7     
\end{tabular}
\caption{Overview of used parameter sets for the CEV, Heston and Merton model}
\label{Tab_Parameters_Pricing}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for CEV
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for CEV}
The CEV model consists of two parameters. Similar to the Black-Scholes model there is a constant parameter $\sigma$ which scales the volatility of the underlying. The main feature of the CEV model is the elasticity of variance parameter $\zeta$ which is combined with the level of the underlying to achieve a non-constant, local volatility, namely $\sigma(S,t)=\sigma S^{\zeta-1}$.  The elasticity of variance parameter is fixed to $0<\zeta<1$ and therefore meant to capture the in practice observable leverage effect. This means when the stock price decreases the volatility usually increases. In this study we want to analyze what effect this local volatility has for American option prices and how strong the De-Americanization effect is depending on value of the elasticity parameter $\zeta$ . If we set $\zeta=1$ we are in the Black-Scholes model. Thus, our selection for $\zeta$ in $p_1$ is 0.5, thus strongly differing from the Black-Scholes model and then $\zeta$ is increasing further until 0.9 within the scenarios. Additionally, we increase the $\sigma-$value in the scenarios to cover a reliable range.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for Heston
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for Heston}
In contrast to the CEV model, which covers the leverage effect by a local volatility function, the main feature of the Heston model is a second stochastic process to describe the volatility. In general %\todo{add sources} 
for stocks the correlation between the volatility and the underlying value is negative. Thus, we focus in the De-Americanization study on negative correlation values $\rho$. Starting in $p_1$ with a scenario in which the volatility is relatively low and the correlation $\rho$ is slightly negative, we increase in $p_2$ to $p_4$ the volatility of volatility parameter $\xi$ and accordingly increase the mean reverting level $\gamma$ and the mean reverting speed $\kappa$ as well as investigate higher negative values for the correlation $\rho$. In all scenarios the initial volatility $v_0$ is set to match the mean reverting level, i.e. $v_0=\gamma$.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for CEV
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for the Merton model}
The Merton model is a jump diffusion model. Due to the early exercise feature of American options, the existence of jumps has a significant impact on American option prices. Consider for example an American put. Here, the option holder benefits from decreasing asset prices. Consequently, when the possibility of negative jumps increases the option price will increase as well. The jump intensity parameter $\lambda$ therefore plays a decisive role in this De-Americanization study. The analogous reasoning holds for the expected jump size parameter $\alpha$. In the upcoming analysis we try to incorporate these effects. The considered scenarios for the Merton model presented in Table~\ref{Tab_Parameters_Pricing} are chosen by this reasoning. Scenario $p_1$ describes a rather Black-Scholes like market with a rather low presence of jump occurrences. In Scenario $p_2$ and $p_3$ the jump feature appears more pronounced. Scenario $p_4$ and $p_5$ finally are encoded by rather jump dominated parameter sets an expected number of $7$ jumps per year with large expected negative jump sizes that appear highly volatile.


%% Absatz zur Selektion der De-Americanized Daten, Amerikanischer Put-Preis muss in continuation region liegen, d.h. P_Am >=max(K-S,0)*(1+delta), delta =0.01
\begin{remark}\label{Remark_Exercise_Region}
In this pricing exercise we price the put options in (\ref{DeAm_Pricing_Setting}) for the parameter sets shown in Table \ref{Tab_Parameters_Pricing}. For some parameters, especially high interest rates combined with low volatility, it could occur that the price of an American put option equals exactly $K_i-S_0$, thus this American put option would be exercised immediately. In the following analysis we excluded these cases because by applying the binomial tree an unique European option price couldn't be determined. As illustrated in the following toy example in Figure \ref{Toy_Example}, there are several values for $u$ possible to replicate the American option price if the price of the American option is given by immediate exercise. In the example, a put option with strike $K=120$ is priced. Here, $u=1.04$ and $u=1.11$ are possible solutions. To avoid this we consequently consider in our analyses only American put options when $P_{Am}>(K-S_0)^{+}\cdot (1+\delta)$. Thus, the American put option price exceeds the immediate exercise price by a factor $\delta$. We set $\delta=1 \%$.  
\begin{figure}
 \centering  
  \begin{minipage}{0.8\textwidth} 
     \centering 
     \includegraphics[width=0.8\textwidth]{./fig/TreeToy_v1.jpg} 
 \end{minipage} 
   \begin{minipage}{0.8\textwidth} 
     \centering 
     \includegraphics[width=0.8\textwidth]{./fig/TreeToy_v2.jpg} 
 \end{minipage}
  \caption{Given an American put option price of 20 with $S_0=100$, $K=120$, $r=0.01$, thus an American put option in the exercise region, an unique tree can't be found to replicate this option. In this example, $u=1.04$ (top) as well as $u=1.11$ (bottom) replicate the American option price but result in different European put prices: 18.81 resp. 19.69.}
  \label{Toy_Example} 
\end{figure} 
\end{remark}
The observations for each model are shown in Table \ref{Tab_Pricing_CEV} (CEV model), Table \ref{Tab_Pricing_Heston} (Heston model) and in Table \ref{Tab_Pricing_Merton} (Merton model). In these tables we show
\begin{itemize}  
\item the average error $\frac{1}{n}\sum_{i=1}^n Price_{DeAm}^i-Price_{EU}^i$
\item the maximal absolute error $max_{i=1}^n Price_{DeAm}^i-Price_{EU}^i$ 
\item the maximal price $max_{i=1}^n Price_{EU}^i$ to reflect the issue stated in Remark \ref{Remark_Exercise_Region}.
\end{itemize} 
In general, we observe for the CEV model, that for short maturities the de--americanized prices seem to overprice the European prices whereas for longer maturities they seem to underprice the European options. In our test settings the switch from underpricing to overpricing depends on the parameter set. By looking at the maximal absolute error we see, that with increasing $\sigma$ and $\zeta$ parameters the maximal error increases. Regarding the average error, all parameter sets behave similarly. Focusing on the interest rate, we observe that for higher interest rates ($r=5\%$ and $r=7\%$) the average error and the maximal error are higher or at least in a comparable region. Especially for higher interest rates the maximal price has to be considered, because the higher the interest rate gets, the higher is the probability that we did not consider some in-the-money options due to Remark \ref{Remark_Exercise_Region} and that the options with high prices are neglected in this setting. Thus we can deduct, that the error increases with increasing interest rates and that at high maturities the error increases for scenarios with higher volatility.\\
For the Heston model we observe in general that the De--Ameri\-cani\-za\-tion error increases with increasing interest rates within each parameter setting. Additionally we see, that for $r=0\%$ there is hardly any effect. By focusing on the scenarios with a higher volatility of volatility parameter ($p_4$ and $p_5$), we observe stronger De--Ameri\-cani\-za\-tion effects at short and long maturities ($T_1$ and $T_2$). Consistently through all scenarios for short maturities the de--americanized price is lower than the according European price whereas for high maturities the de--americanized price is higher than the according European price.\\
For the Merton model we observe similar, little effects for scenarios $p_1$ and $p_2$, i.e. the scenarios with low jump intensity, whereas for the scenarios with increasing jump intensity ($p_3$, $p_4$ and $p_5$) we observe stronger De--Ameri\-cani\-za\-tion effects especially for increasing maturities and interest rates.
%The only question, that is not been answered by Table \ref{Tab_Pricing_CEV}, is the question if there are different effects for in-the-money and out-of-the money options. For illustration purposes Figure \ref{Fig_Pricing_CEV} visualizes the results for parameter set $p_i$ and \todo{add figure and number parameter set} interest rate $r=x\%$. \todo{Interpretation Figure}
%For the Heston model we observe that for short maturities the de--americanized prices seem to underprice, whereas for increasing maturities they seem to overprice. More interestingly, for increasing interest rates tend to lead to overpriced de--americanized prices. Accordingly, here Figure \ref{Fig_Pricing_Heston}\todo{Figure einbauen}. 



\input{./tex/table_pricing}
\input{./tex/table_pricing_heston}
\input{./tex/table_pricing_merton}



\subsection{Effects of De--Ameri\-cani\-za\-tion on Calibration to Synthetic Data}
\label{sec:Calibration_Synthetic}

We study the De-Americanization effect on synthetic American market data. To this extent, in a first step we generate artificial market data using our FEM implementations of the three considered models. In a second step we calibrate each model to the previously generated market data. This methodology allows disregarding the noise that real market data is affiliated with and thus permits studying the De-Americanization effect exlusively.\\

Our artificial market data is specified as follows.
\begin{equation}
\begin{alignedat}{2}
S_0&=1\\
r&=7\%\\
T_1&=\frac{2}{12},\qquad &&K_1=\{0.95, 0.975, 1, 1.025, 1.05\},\\
T_2&=\frac{6}{12},\qquad &&K_2=\{0.9,0.925,K_1,1.075,1.1\},\\
T_3&=\frac{9}{12},\qquad &&K_3=\{0.85,0.875,K_2,1.125,1.15\},\\
T_4&=1,\qquad &&K_4=\{0.8,0.825,K_3,1.175,1.2\},\\
T_5&=2,\qquad &&K_5=\{0.75, 0.775, K_4,1.225,1.25\}.
\end{alignedat}
\label{eq:syndatasetting}
\end{equation}

As the data in~\eqref{eq:syndatasetting} shows, we consider a high-interest market and a set of maturities ranging from rather short-term American options of 2 months before maturity to long-term American products of 2 years before maturity. Each maturity $T_i$ is associated with a set of strikes $K_i$, $i\in\{1,\dots,5\}$. As for the analysis of De--Ameri\-cani\-za\-tion effects on pricing, we price these options for the five parameter scenarios in Table \ref{Tab_Parameters_Pricing}. Regarding the calibration methodology, we have to make two choices. First we have to decide which option types do we include and second how the objective function looks like.

Regarding the choice of options we first consider only Put options for the whole strike trajectory. Thus, we include in-the-money as well as out-of-the-money options. Second, driven by the fact that the value of out-of-the-money options does not include any intrinsic value and is therefore supposed to reflect the randomness of the market better,%\todo{Reference}
we consider as a second approach to only include out-of-the money puts and out-of-the money calls for the whole set of strikes and maturities. Consequently, in this second study for each $i\in\{1,\dots,5\}$ we consider call option prices for maturities $T_i$ and strikes $k\in K_i$ with $k>1$ and put option prices for maturities $T_i$ and strikes $k\in K_i$ with $k<1$. At-the-money option data, i.e. options with strike $K=1$ is neglected.

Once the American market has been generated, we create an associated second market by applying the De-Americanization routine using the tree model. We thus deamericanize each price individually by calibrating the tree model first and then deriving the associated quasi-European deamericanized price.

Remark~\ref{Remark_Exercise_Region} and Figure~\ref{Toy_Example} described situations in which the De-Americanization routine yields non-unique results. In the calibration to de-Americanized prices we exclude those options that can not be deamericanized uniquely as the following remark underpins.

\begin{remark}[Disregarding non-unique deamericanized prices]
\label{rem:PutOptionsOutinCalib}
As outlined above, we artificially generate American market data for a calibration study on synthetic data. In a first step we calibrate to the generated American prices directly. Here, all generated data is considered. In a second step, we deamericanize the option data and calibrate to the resulting quasi-European options. Here, only those option prices are considered that allow for a unique deamericanized price. Consequently, all American put option prices that violate
	\begin{equation}
	\label{cond:DisregardAtCalib}
		P^\text{put}_{Am}>(K-S_0)^{+}\cdot (1+\delta),\qquad \text{ with } \delta=1 \%,
	\end{equation}
are not de-americanized and thus neglected in the second step.
\end{remark}

The second critical assumption is the objective function. A variety of objective functions is proposed in the literature,e.g. the root mean square error, the average absolute error as a percentage of the mean price, the average absolute error, the average relative percentage error, absolute price differences, relative price differences, absolute implied volatilities, relative implied volatilities (e.g. \cite{detlefsenhaerdle}, \cite{bauer}, \cite{fengler}, \cite{schoutens}).

In the calibration, we take the absolute average squared error (aase) as an objective function and thus minimize
\begin{equation}
\text{aase}=\frac{1}{\#\text{options}}\sum_{\text{option}_k}\vert \text{Market price}_k-\text{Model price}_k\vert^2.\label{objectivefunction}
\end{equation}

The results of the calibration to synthetic data are summarized in Table \ref{Tab_Calibration_Synthetic_Data_Put} for calibrating to put options and in Table \ref{Tab_Calibration_Synthetic_Data_oom} for calibrating to out-of-the-money options.\todo{Note: CEV result not final}

\input{./tex/table_calibration_put}
\input{./tex/table_calibration_oom}
\input{./tex/table_google}
Overall we see that for the CEV model that by calibrating to American options, the parameters more or less match. By calibrating to de-americanized prices however, the volatility parameter $\sigma$ is in most of the cases underestimated and this underestimation is captured by an overestimated $\zeta$ value.

Focusing on the Heston model, we observe that in all calibration to American options the parameters are matched. Comparing calibration results with the according calibration to de--ameri\-cani\-zed data, we clearly see that the three parameters $\gamma$, $\kappa$ and $v_0$ are matched, but the remaining two parameters $\xi$ and $\rho$ show different results. By calibrating to put options, with increasing volatility of volatility parameters $\xi$ the calibrated de--ameri\-cani\-zed parameter overestimates the true parameter. By calibrating to out-of-the-money options, we observe for $\xi$ an underestimation for lower $\xi$ values and an overestimation for higher $\xi$ values. Regarding $\rho$, with increasing volatility of volatility the de--ameri\-cani\-zed parameter tends to underestimate the $\rho$ value. By focusing later on pricing exotic options, we will see whether these two contrary effects will cancel each other or lead to different exotic option prices.\\
For the Merton model we observe the general picture, that by calibrating to American options $\sigma$ is matched. For the other 3 parameters we observe that whenever the jump intensity $\lambda$ is underestimated the according mean $\alpha$ and standard deviation $\beta$ of the jump are adjusted accordingly. Similar observation can be made for calibration to de--ameri\-cani\-zed prices. Here, especially for calibration to out-of-the-money values in $p_4$ and $p_5$ we observe that the $\sigma$ value is additionally not matched.

\subsection{Effects of De--Ameri\-cani\-za\-tion on Calibration to Market Data}
%\label{sec:Calibration_Market}
In order to structure the available data, we follow the methodology applied for the volatility index (VIX) by the Chicago board of exchange (\cite{vix}):
\begin{itemize}
\item Only out-of-the-money put and call options are used
\item The midpoint of the bid-ask spread for each option with strike $K_i$ is considered 
\item Only options with non-zero bid prices are considered
\item Once two puts with consecutive strike prices are found to have zero bid
prices, no puts with lower strikes are considered for inclusion (same for calls)
\end{itemize}
Basically, by this selection procedure, we only select out-of-the-money options that (due to non-zero bid prices) can be considered as liquid. In general, an option price consists of two components reflecting the time value and the intrinsic value of the option. By focusing on out-of-the-money options intrinsic value effects are mostly neglected and the highest option price will be at-the-money. Additionally, the highest market activity is in the at-the-money and slightly out-of-the-money region. 
The calibration results are summarized in Table \ref{Tab_Calibration_Google}\todo{Note: CEV result not final} and illustrated in Figures \ref{Figure_Google_CEV2}, \ref{Figure_Google_Heston2} and \ref{Figure_Google_Merton}. 
\begin{figure}
 \centering 
     \includegraphics[width=\textwidth]{./fig/Google_CEV.jpg}    
     \caption{CEV calibration results of calibrating to Google market data.} 
      \label{Figure_Google_CEV2}
\end{figure}

\begin{figure}
 \centering 
     \includegraphics[width=\textwidth]{./fig/Google_Heston.png}     
     \caption{Heston calibration results of calibrating to Google market data.} 
     \label{Figure_Google_Heston2}
\end{figure}

%\begin{figure}
% \centering 
%    % \includegraphics[width=\textwidth]{./fig/Google_Merton.jpg}
%     \label{Figure_Google_Merton}
%     \caption{Merton calibration results of calibrating to Google market data.} 
%\end{figure}

Here we observe hardly any differences in the parameters. This is most likely due to the low interest rate environment. In this settings, American and European puts coincide and thus, there will hardly be any difference in the prices and thus it is rather normal that we observe similar calibration results.

\subsection{Effects of De--Ameri\-cani\-za\-tion in pricing exotic options}

In the market plain vanilla option prices are traded liquidly and these prices are used to calibrate models. That's what has been done in the previous subsections. But financial institutions are interested in pricing more exotic products like e.g. barrier and lookback options. In this subsection we analyze a down-and-out call option and a lookback option and therewith translate differences in the calibrated models into quantitative prices. The payoff $p(S(T))$ of a down-and-out call option with barrier $B$ is given by
\begin{align}
p(S(T))=(S(T)-K)^{+}\cdot\mathbbm{1}_{\min_{t\le T}S(t)\ge B}. 
\end{align}
For our setting we set $S_0=100$, the barrier $B$ to 90\% of the initial underlying value, $B=0.9\cdot S(0)$ and the strike $K$ to 105\% of the underlying value, $K=1.05S(0)$. For a lookback option we choose the same strike and the payoff $p(S(T))$ is
\begin{align}
p(S(T))=(\bar{S}(T)-K)^{+},\quad with\ \bar{S}(T)=\max_{t\le T}S(t)
\end{align}

And then we priced the exotic options for the parameters in Tables \ref{Tab_Calibration_Synthetic_Data_Put}, \ref{Tab_Calibration_Synthetic_Data_oom} and \ref{Tab_Calibration_Google}. The results are shown in the following Table \ref{Tab_Exotics}.
\input{./tex/table_exotics}
Overall, we observe an different picture through the three models.

In $p_1$ and $p_2$, the scenarios with relatively small volatility we don't see any differences. Thus in case of a small volatility and a medium elasticity of variance $\zeta$ De--Ameri\-cani\-za\-tion seems to work. In the other scenarios we observe that the calibration to de-americanized prices leads to higher exotic option prices if we calibrate to put options only and lower exotic option prices if we calibrate to out-of-the-money options. Thus, the in general lower calibrated $\sigma$ value in combination with an increased $\zeta$ value by calibrating to de-americanized options has this effect in pricing exotic options.

For the Heston model we see that in the cases when the calibration to de-americanized data led to different $\xi$ and $\rho$ values, there are differences in the exotic option prices. More precisely, in all these cases the according barrier and lookback prices are too high. This means that De--Ameri\-cani\-za\-tion causes an systematic overpricing of exotic options.

For the Merton model we see rather small differences for lookback options, but more interestingly, for the down-and-out barrier option we observe differences. This reflects that the different calibrated jump intensity and accordingly adjusted mean and standard deviation of the jumps can buffer De--Ameri\-cani\-za\-tion over the paths when the option can not vanish like in the barrier option case.

Summarizing the results, we see that De--Ameri\-cani\-za\-tion effect matter and can influence the prices of exotic options. Especially, when the assumed model includes jumps. Thus, if available plain vanilla data is of American type, we recommend a direct calibration to American options. However, the computational costs in this case can be an issue. To overcome it, we present a short overview of a model reduction technique, as a reduced basis method (RBM). That is, we substitute the FEM discrete model with the reduced one, which is much cheaper to compute. Then a whole calibration routine is carried out on a reduced system. Of course, the price to pay is the decreased accuracy of the reduced solution compared to the FEM one. However, in the numerical experiments we observe, that these differences have a little influence on the exactness of the calibrated parameter. Several scenarios can be developed with the use of the RBM strategy. For instance, one can start a calibration routine with RBM and later use the calibrated parameter as an initial guess for the calibration process with FEM. In this way, the RBM calibration would lead us relatively fast to the region of local minimum and, hence, the calibration with the FEM afterwards should terminate relatively quickly. 


  

==> tex/abstract.tex <==
\begin{abstract}
A common approach to calibrate a model on market data involving American options
called De--Ameri\-cani\-za\-tion is investigated. Instead of calibrating market
models to American option prices directly, which is very time-consuming and
often numerically much more demanding - if possible at all, the American option
prices are de-americanized first: One calibrates a simple tree model and then
using the calibrated tree model generates respective European option prices. 
Then models can be calibrated to these pseudo-European option prices. The effect
of this approximation is tested for the CEV, the Heston and the Merton models.
By direct calibration to American option prices we conduct comparisons to the
De-Americanization approach. Both, scenarios where the practitioners'
approximation makes sense and cases where the routine generates unsatisfactory
results are described. \new{In addition we present the reduced basis methods, as
a
model order reduction technique, which allows to achieve a significant speed up
and reduction of the computation complexity of the calibration routine.}
	\end{abstract}
\minisec{Keywords}
	American options, calibration, binomial tree model, CEV model, Heston
model, L\'evy models, finite element methods, \new{model reduction, reduced
basis methods, variational inequalities}

==> tex/calibration.tex <==
\section{Market Data}
\label{calibration_methodology}
Our main aspect is to investigate the De--Ameri\-cani\-za\-tion methodology with respect to real market data. As single stock we have chosen Google. This is due the fact that Google has not paid dividends so far and therefore, we can exclude dividend payments and have to solely work with solvers for non-dividend paying assets. As market data we took delayed quotes from the Chicago Board of exchange.\footnote{http://www.cboe.com/delayedquote/quotetable.aspx, ticker: GOOG}

By selecting the available market data for Google options, overall 1182 options for 7 maturities have been collected. Here, the natural question arises if there are methodologies to select subsets of this data for the calibration procedure.\\
In order to structure the available data, we follow the methodology applied for the volatility index (VIX) by the Chicago board of exchange (\cite{vix}):
\begin{itemize}
\item Only out-of-the-money put and call options are used
\item The midpoint of the bid-ask spread for each option with strike $K_i$ is considered 
\item Only options with non-zero bid prices are considered
\item Once two puts with consecutive strike prices are found to have zero bid
prices, no puts with lower strikes are considered for inclusion (same for calls)
\end{itemize}
Basically, by this selection procedure, we only select out-of-the-money options that (due to non-zero bis prices) can be considered as liquid. In general, an option price consists of two components reflecting the time value and the intrinsic value of the option. By focusing on out-of-the-money options intrinsic value effects are mostly neglected and the highest option price will be at-the-money. Additionally, the highest market activity is in the at-the-money and slightly out-of-the-money region. Overall, Table \ref{GoogleDaten} gives an overview of the processed data for the calibration procedure, in total we achieved a data set containing 482 options, slightly more puts than calls. The risk-free interest rate for maturities 1 month, 3 month, 6 month, 1 year and 2 years are taken from the U.S. Department of the Treasury\footnote{http://www.treasury.gov/resource-center/data-chart-center/interest-rates/Pages/TextView.aspx?data=yield} and have been linearly interpolated whenever necessary. 

\begin{table}[h]
\begin{center}
 \begin{tabular}{|c|c|c|c|c|}
 	\hline
  &Maturity&T&\# of options&r\\
  \hline
  $T_1$&27.02.2015&0.07&47&0.0001\\
    \hline
  $T_2$&20.03.2015&0.13&49&0.000129508\\
    \hline
  $T_3$&17.04.2015&0.20&52&0.00017541\\
    \hline
  $T_4$&19.06.2015&0.38&87&0.00046087\\
    \hline
  $T_5$&18.09.2015&0.62&98&0.000955435\\
    \hline
  $T_6$&15.01.2016&0.95&101&0.001602174\\
    \hline
  $T_7$&20.01.2017&1.97&48&0.004786339\\
  \hline
 \end{tabular}
 \caption{Processed Google option data for $t_0=\text{02.02.2015}$, $S_0=523.76$}
 \label{GoogleDaten}
 \end{center}
\end{table}


Regarding calibration, one critical assumption is the objective function. A variety of objective functions is proposed in the literature,e.g. the root mean square error, the average absolute error as a percentage of the mean price, the average absolute error, the average relative percentage error, absolute price differences, relative price differences, absolute implied volatilities, relative implied volatilities (e.g. \cite{detlefsenhaerdle}, \cite{bauer}, \cite{fengler}, \cite{schoutens}).

In the calibration, we focus in the following on the absolute pricing error (ape):
\begin{equation}
ape=\frac{1}{number\ of\ options}\sum_{options}\vert Market\ price-Model\ price\vert^2\label{objectivefunction}
\end{equation}
%%

==> tex/conclusion.tex <==
\section{Conclusion}
In this paper we investigated the De--Ameri\-cani\-za\-tion method for local volatility, stochastic volatility and a jump-diffusion model.\\

\begin{itemize}
\item Pricing:
\begin{itemize}
\item CEV
\begin{itemize}
\item increases with increasing interest rates and that at high maturities the error increases for scenarios with higher volatility
\end{itemize}
\item Heston
\begin{itemize}
\item De--Ameri\-cani\-za\-tion error increases with increasing interest rates.
\item Additionally we see, that for $r=0\%$ there is hardly any effect.
\item By focusing on the scenarios with a higher volatility of volatility parameter ($p_4$ and $p_5$), we observe stronger De--Ameri\-cani\-za\-tion effects at short and long maturities ($T_1$ and $T_2$)
\item For short maturities the de--americanized price is lower than the according European price whereas for high maturities the de--americanized price is higher than the according European price.
\end{itemize}
\item Merton
\begin{itemize}
\item Little effects for scenarios with low jump intensity
\item For the scenarios with increasing jump intensity ($p_3$, $p_4$ and $p_5$) we observe stronger De--Ameri\-cani\-za\-tion effects especially for increasing maturities and interest rates.
\end{itemize}
 \end{itemize}
\item Calibration to synthetic data:
\begin{itemize}
\item CEV: In general $\sigma$ is underestimated and $\rho$ overestimated by calibrating to de-americanized data
\item Heston: In general $\xi$ and $\rho$ are critical parameters which are calibrated differently by calibrating to de-americanized data
\item Merton: In general, jump intensity $\lambda$ is underestimated and this is compensated by higher values for the mean and standard deviation of the jump
\end{itemize}
\item Calibration to Google data: 
\begin{itemize}
\item Hardly any different calibration results. This is due to low interest environment
\end{itemize}
\item Pricing exotic options:
\begin{itemize}
\item CEV: Underestimated $\sigma$ and $\rho$ values of calibrating to de-americanized prices lead to hgiher or lower exotic option prices.
\item Heston: Due to different $\xi$ and $\rho$ values, we observe big differences in exotic option prices.
\item Merton: Differences for barrier option, only little differences for lookbacks, i.e. different jump intensities can be compensated over the path (lookback) with different mean and standard deviation of the jump, but the critical aspect of an vanishing option (barrier) is not covered sufficiently
\end{itemize}
\item Outlook RB introduces RB to speed up calibration process
\end{itemize} 

==> tex/numerical_study1.tex <==
\section{Numerical Study of De--Ameri\-cani\-za\-tion effects} 
Our main objective is to investigate the De--Ameri\-cani\-za\-tion methodology with respect to calibration. How accurate does this methodology work and if there are differences, how crucial are these. But before we look at calibration in detail, we present an accuracy study of our FEM pricers followed by an investigation of De--Ameri\-cani\-za\-tion effects on pricing. Then we switch to calibration to synthetic data and finally, market data.

\subsection{Accuracy Study}
Here we investigate the accuracy of our FEM solvers for the previously presented models for European options. Therefore, we define a test scenario of put and call options and illustrate the errors compared to benchmark solutions. %More specifically, we only investigate here out-of-the-money options because later in the calibration methodology only out-of-the-money options are considered. \todo{oom options too short?} 
In our test setting we set $S_0=1$, $r=0.07$, $T=\{0.5,0.875, 1.25, 1.625,2\}$ and we set $K$ to 21 equally distributed values in $[0.5,1.5]$. For the discretization we set $[S_min,S_max]=[0.01,2]$ for the CEV model, $[v_{min}, v_{max}]=[10^{-5},3]$ and  $[x_{min}, x_{max}]=[-5,5]$ for the Heston model and for the Merton model we set $[x_{min}, x_{max}]=[,]$. We set $\mathcal{N}=1000$ for the CEV model, $\mathcal{N}=49\times 97=4753$ for the Heston model and for the Merton model $\mathcal{N}=$, and $\Delta t = 0.008$ for all models.

Figure \ref{Accuracy_CEV_Puts} illustrates the accuracy results for put options in the CEV model. Here, we choose model parameters $\sigma=0.15$ and $\rho=0.75$ and as benchmark solution we implemented the closed-form solution of the CEV model for European put and call prices as shown in \cite{schroeder}. Overall, we observe that the absolute errors are in the $10^{-4}$ region. Naturally, we observe that in-the-money occur the highest option prices and the prices decrease in the out-of-money directions. Figure \ref{Accuracy_CEV_Puts} shows the results for call options. By comparing put and call prices we see, that the call prices are higher than the put prices which can be explained by the locally on the underlying value depending volatility. 
Furthermore we observe that the absolute error between benchmark and FEM solutions increases slightly with increasing maturities.
% and that for put options the error is the highest in the close to at-the-money region, whereas for call options the error by going further out-of-the-money first increases, peaks at $K=1.2$ to $K=1.3$ and then decreases again.
\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Puts_Price.jpg} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Puts_Diffs.jpg} 
  \end{minipage} 
  \caption{Accuracy study for put options in the CEV model. Option prices (left) and absolute differences between benchmark and FEM solution (right)}
  \label{Accuracy_CEV_Puts} 
\end{figure} 

\begin{figure} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Call_Prices.jpg} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/Acc_Call_Diffs.jpg} 
  \end{minipage} 
  \caption{Accuracy study for call options in the CEV model. Option prices (left) and absolute differences between benchmark and FEM solution (right)}
  \label{Accuracy_CEV_Calls} 
\end{figure} 
%
%%  %%%%%%%%%%%%%%%%%% Heston model accuracy %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
For the Heston model we used the closed-form solution in~\citep{janek2011fx} as benchmark. As model parameters we use $\parmu=(0.1, -0.5, 0.05, 1.2, 0.001)$ with $v_0=0.05$. The accuracy results for put and call options using a closed-form solution are summarized in Figure~\ref{Accuracy_Heston_Semi_put} and Figure~\ref{Accuracy_Heston_Semi_call} respectively. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Heston (put)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h!]
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_put_winkl10_dt008_DOF18721_FourSOL}
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_put_winkl10_dt008_DOF18721_FourDIF} 
%     \caption{Accuracy study for put options in the Heston model. Left: Option prices obtained using the Fourier method (circles) and the FEM method (stars). Right: The respective absolute differences.}
%     \label{Heston_Fourier_put}
%   \end{figure}    

\begin{figure}[h!]    
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_put_stand10_dt008_DOF4753_SemiSOL.png}
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_put_stand10_dt008_DOF4753_SemiDIF.png} 
     \caption{Accuracy study for put options in the Heston model. Left: Option prices obtained with the semiclosed formula (circles) and the FEM method (stars). Right: The respective absolute differences.}
     \label{Accuracy_Heston_Semi_put}
   \end{figure}    


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Heston (call)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h!]
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_call_winkl10_dt008_DOF18721_FourSOL}
%     \includegraphics[width=.5\textwidth]{./fig/heston/24Nov15_market_semianalytic8_call_winkl10_dt008_DOF18721_FourDIF} 
%     \caption{Accuracy study for call options in the Heston model. Left: Option prices obtained using the Fourier method (circles) and the FEM method (stars). Right: The respective absolute differences.}
%      \label{Heston_Fourier_call}
%   \end{figure}    

\begin{figure}[h!]   
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_call_stand10_dt008_DOF4753_SemiSOL.png}
     \includegraphics[width=.5\textwidth]{./fig/heston/05Feb16_market_semianalytic_stmesh_call_stand10_dt008_DOF4753_SemiDIF.png} 
     \caption{Accuracy study for call options in the Heston model. Left: Option prices obtained with the semiclosed formula (circles) and the FEM method (stars). Right: The respective absolute differences.} \label{Accuracy_Heston_Semi_call}
   \end{figure}    


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Lastly, Figure~\ref{fig:Accuracy_Merton_Puts} shows the results for European put options and Figure~\ref{fig:Accuracy_Merton_Calls} shows the results for European call options in the Merton model. Here, Fourier pricing is used as benchmark. For this accuracy study, the model is parametrized setting $\sigma=0.2$, $\alpha=-0.1$, $\beta=0.1$ and $\lambda=3$. In both figures, the interest rate $r$ has been chosen at a rather high rate, $r=7\%$. Similarly to the previous models the error is in the $10^{-4}$ region. In contrast, we observe that the error decreases with increasing maturities except in the deep out-of-the-money regions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Merton (put)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_putcloudpic} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_putAbsDiff} 
  \end{minipage} 
  \caption{Accuracy study for put options in the Merton model. Left: Option prices from the reference method (circles) and the FEM method (stars). Right: The respective absolute differences.}
  \label{fig:Accuracy_Merton_Puts} 
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fig. Accuracy Study Merton (call)
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_callcloudpic} 
 \end{minipage} 
  \begin{minipage}{0.49\textwidth} 
     \centering 
     \includegraphics[width=\textwidth]{./fig/max/Accuracy/Merton_callAbsDiff} 
  \end{minipage} 
  \caption{Accuracy study for call options in the Merton model. Left: Option prices from the reference method (circles) and the FEM method (stars). Right: The respective absolute differences.}
  \label{fig:Accuracy_Merton_Calls} 
\end{figure} 

Summarizing the accuracy study, we observe that for all models the absolute error between benchmark and FEM solution is in the $10^{-3}$ to the $10^{-4}$ region.

\subsection{Effects of De--Ameri\-cani\-za\-tion on Pricing}
\label{sec:Pricing}

After we have presented our models, we want to firstly focus on differences caused by the De--Ameri\-cani\-za\-tion itself. Therefore, we compare de--americanized American prices with derived European option prices as illustrated in Figure \ref{DeAmPricing} and analyze the differences. 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/DeAmPricing.png}
\caption{First Step De--Ameri\-cani\-za\-tion: Focus on pricing differences}
\label{DeAmPricing}
\end{center}
\end{figure}

The advantage of this approach is that we can purely focus on the De--Ameri\-cani\-za\-tion without mixing it with any calibration issues. In order to do so, we defined the following test set for the range of investigated options. Here we focus on put options due to the fact that non dividend payments lead to the same prices for American and European calls.
\begin{align}
S_0&=1\notag\\
K&=0.80,0.85,0.90,0.95,1.00,1.05,1.10,1.15,1.20\notag\\
T&=\frac{1}{12},\frac{2}{12},\frac{3}{12},\frac{4}{12},\frac{6}{12},\frac{9}{12},\frac{12}{12},\frac{24}{12}\notag\\
r&=0, 0.01, 0.02, 0.05,0.07\label{DeAm_Pricing_Setting}
\end{align}
In each model, 5 parameter sets are investigated to cover the parameter range. These are summarized in Table \ref{Tab_Parameters_Pricing}. 
\begin{table}[h!]
\centering
\begin{tabular}{ccc|ccccc|cccc}
      & \multicolumn{2}{c|}{CEV} & \multicolumn{5}{c|}{Heston}                    & \multicolumn{4}{c}{Merton} \\
      & $\sigma$   & $\xi$ & $\zeta$ & $\rho$ & $\gamma$ & $\kappa$ & $v_0$ & $\sigma$ & $\alpha$    & $\beta$    & $\lambda$ \\ \hline
$p_1$ & $0.2$      & $0.5$ & 0.10     & -0.20      & 0.07     & 0.1      & 0.07  & 0.20      &  -0.01      & 0.01       & 1 \\
$p_2$ & $0.275$    & $0.6$ & 0.25     & -0.50   & 0.10     & 0.4      & 0.10  & 0.15     &  -0.05      & 0.05       & 2 \\
$p_3$ & $0.35$     & $0.7$ & 0.40     & -0.50    & 0.15     & 0.6      & 0.15  & 0.20      &  -0.10       & 0.10        & 3 \\
$p_4$ & $0.425$    & $0.8$ & 0.55     & -0.45   & 0.20     & 1.2      & 0.20  & 0.10      &  -0.10       & 0.20        & 5 \\
$p_5$ & $0.5$      & $0.9$ & 0.70     & -0.80    & 0.30      & 1.4      & 0.30  & 0.10      &  -0.15      & 0.20        & 7     
\end{tabular}
\caption{Overview of used parameter sets for the CEV, Heston and Merton model}
\label{Tab_Parameters_Pricing}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for CEV
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for CEV}
The CEV model consists of two parameters. Similar to the Black-Scholes model there is a constant parameter $\sigma$ which scales the volatility of the underlying. The main feature of the CEV model is the elasticity of variance parameter $\zeta$ which is combined with the level of the underlying to achieve a non-constant, local volatility, namely $\sigma(S,t)=\sigma S^{\zeta-1}$.  The elasticity of variance parameter is fixed to $0<\zeta<1$ and therefore meant to capture the in practice observable leverage effect. This means when the stock price decreases the volatility usually increases. In this study we want to analyze what effect this local volatility has for American option prices and how strong the De-Americanization effect is depending on value of the elasticity parameter $\zeta$ . If we set $\zeta=1$ we are in the Black-Scholes model. Thus, our selection for $\zeta$ in $p_1$ is 0.5, thus strongly differing from the Black-Scholes model and then $\zeta$ is increasing further until 0.9 within the scenarios. Additionally, we increase the $\sigma-$value in the scenarios to cover a reliable range.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for Heston
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for Heston}
In contrast to the CEV model, which covers the leverage effect by a local volatility function, the main feature of the Heston model is a second stochastic process to describe the volatility. In general %\todo{add sources} 
for stocks the correlation between the volatility and the underlying value is negative. Thus, we focus in the De-Americanization study on negative correlation values $\rho$. Starting in $p_1$ with a scenario in which the volatility is relatively low and the correlation $\rho$ is slightly negative, we increase in $p_2$ to $p_4$ the volatility of volatility parameter $\xi$ and accordingly increase the mean reverting level $\gamma$ and the mean reverting speed $\kappa$ as well as investigate higher negative values for the correlation $\rho$. In all scenarios the initial volatility $v_0$ is set to match the mean reverting level, i.e. $v_0=\gamma$.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Rem.: Motivation of parameter selection for CEV
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Motivation of parameter selection for the Merton model}
The Merton model is a jump diffusion model. Due to the early exercise feature of American options, the existence of jumps has a significant impact on American option prices. Consider for example an American put. Here, the option holder benefits from decreasing asset prices. Consequently, when the possibility of negative jumps increases the option price will increase as well. The jump intensity parameter $\lambda$ therefore plays a decisive role in this De-Americanization study. The analogous reasoning holds for the expected jump size parameter $\alpha$. In the upcoming analysis we try to incorporate these effects. The considered scenarios for the Merton model presented in Table~\ref{Tab_Parameters_Pricing} are chosen by this reasoning. Scenario $p_1$ describes a rather Black-Scholes like market with a rather low presence of jump occurrences. In Scenario $p_2$ and $p_3$ the jump feature appears more pronounced. Scenario $p_4$ and $p_5$ finally are encoded by rather jump dominated parameter sets an expected number of $7$ jumps per year with large expected negative jump sizes that appear highly volatile.


%% Absatz zur Selektion der De-Americanized Daten, Amerikanischer Put-Preis muss in continuation region liegen, d.h. P_Am >=max(K-S,0)*(1+delta), delta =0.01
\begin{remark}\label{Remark_Exercise_Region}
In this pricing exercise we price the put options in (\ref{DeAm_Pricing_Setting}) for the parameter sets shown in Table \ref{Tab_Parameters_Pricing}. For some parameters, especially high interest rates combined with low volatility, it could occur that the price of an American put option equals exactly $K_i-S_0$, thus this American put option would be exercised immediately. In the following analysis we excluded these cases because by applying the binomial tree an unique European option price couldn't be determined. As illustrated in the following toy example in Figure \ref{Toy_Example}, there are several values for $u$ possible to replicate the American option price if the price of the American option is given by immediate exercise. In the example, a put option with strike $K=120$ is priced. Here, $u=1.04$ and $u=1.11$ are possible solutions. To avoid this we consequently consider in our analyses only American put options when $P_{Am}>(K-S_0)^{+}\cdot (1+\delta)$. Thus, the American put option price exceeds the immediate exercise price by a factor $\delta$. We set $\delta=1 \%$.  
\begin{figure}
 \centering  
  \begin{minipage}{0.8\textwidth} 
     \centering 
     \includegraphics[width=0.8\textwidth]{./fig/TreeToy_v1.jpg} 
 \end{minipage} 
   \begin{minipage}{0.8\textwidth} 
     \centering 
     \includegraphics[width=0.8\textwidth]{./fig/TreeToy_v2.jpg} 
 \end{minipage}
  \caption{Given an American put option price of 20 with $S_0=100$, $K=120$, $r=0.01$, thus an American put option in the exercise region, an unique tree can't be found to replicate this option. In this example, $u=1.04$ (top) as well as $u=1.11$ (bottom) replicate the American option price but result in different European put prices: 18.81 resp. 19.69.}
  \label{Toy_Example} 
\end{figure} 
\end{remark}
The observations for each model are shown in Table \ref{Tab_Pricing_CEV} (CEV model), Table \ref{Tab_Pricing_Heston} (Heston model) and in Table \ref{Tab_Pricing_Merton} (Merton model). In these tables we show
\begin{itemize}  
\item the average error $\frac{1}{n}\sum_{i=1}^n Price_{DeAm}^i-Price_{EU}^i$
\item the maximal absolute error $max_{i=1}^n Price_{DeAm}^i-Price_{EU}^i$ 
\item the maximal price $max_{i=1}^n Price_{EU}^i$ to reflect the issue stated in Remark \ref{Remark_Exercise_Region}.
\end{itemize} 
In general, we observe for the CEV model, that for short maturities the de--americanized prices seem to overprice the European prices whereas for longer maturities they seem to underprice the European options. In our test settings the switch from underpricing to overpricing depends on the parameter set. By looking at the maximal absolute error we see, that with increasing $\sigma$ and $\zeta$ parameters the maximal error increases. Regarding the average error, all parameter sets behave similarly. Focusing on the interest rate, we observe that for higher interest rates ($r=5\%$ and $r=7\%$) the average error and the maximal error are higher or at least in a comparable region. Especially for higher interest rates the maximal price has to be considered, because the higher the interest rate gets, the higher is the probability that we did not consider some in-the-money options due to Remark \ref{Remark_Exercise_Region} and that the options with high prices are neglected in this setting. Thus we can deduct, that the error increases with increasing interest rates and that at high maturities the error increases for scenarios with higher volatility.\\
For the Heston model we observe in general that the De--Ameri\-cani\-za\-tion error increases with increasing interest rates within each parameter setting. Additionally we see, that for $r=0\%$ there is hardly any effect. By focusing on the scenarios with a higher volatility of volatility parameter ($p_4$ and $p_5$), we observe stronger De--Ameri\-cani\-za\-tion effects at short and long maturities ($T_1$ and $T_2$). Consistently through all scenarios for short maturities the de--americanized price is lower than the according European price whereas for high maturities the de--americanized price is higher than the according European price.\\
For the Merton model we observe similar, little effects for scenarios $p_1$ and $p_2$, i.e. the scenarios with low jump intensity, whereas for the scenarios with increasing jump intensity ($p_3$, $p_4$ and $p_5$) we observe stronger De--Ameri\-cani\-za\-tion effects especially for increasing maturities and interest rates.
%The only question, that is not been answered by Table \ref{Tab_Pricing_CEV}, is the question if there are different effects for in-the-money and out-of-the money options. For illustration purposes Figure \ref{Fig_Pricing_CEV} visualizes the results for parameter set $p_i$ and \todo{add figure and number parameter set} interest rate $r=x\%$. \todo{Interpretation Figure}
%For the Heston model we observe that for short maturities the de--americanized prices seem to underprice, whereas for increasing maturities they seem to overprice. More interestingly, for increasing interest rates tend to lead to overpriced de--americanized prices. Accordingly, here Figure \ref{Fig_Pricing_Heston}\todo{Figure einbauen}. 



\input{./tex/table_pricing}
\input{./tex/table_pricing_heston}
\input{./tex/table_pricing_merton}

==> tex/numerical_study2.tex <==




\subsection{Effects of De--Ameri\-cani\-za\-tion on Calibration to Synthetic Data}
\label{sec:Calibration_Synthetic}

We study the De-Americanization effect on synthetic American market data. To this extent, in a first step we generate artificial market data using our FEM implementations of the three considered models. In a second step we calibrate each model to the previously generated market data. This methodology allows disregarding the noise that real market data is affiliated with and thus permits studying the De-Americanization effect exlusively.\\

Our artificial market data is specified as follows.
\begin{equation}
\begin{alignedat}{2}
S_0&=1\\
r&=7\%\\
T_1&=\frac{2}{12},\qquad &&K_1=\{0.95, 0.975, 1, 1.025, 1.05\},\\
T_2&=\frac{6}{12},\qquad &&K_2=\{0.9,0.925,K_1,1.075,1.1\},\\
T_3&=\frac{9}{12},\qquad &&K_3=\{0.85,0.875,K_2,1.125,1.15\},\\
T_4&=1,\qquad &&K_4=\{0.8,0.825,K_3,1.175,1.2\},\\
T_5&=2,\qquad &&K_5=\{0.75, 0.775, K_4,1.225,1.25\}.
\end{alignedat}
\label{eq:syndatasetting}
\end{equation}

As the data in~\eqref{eq:syndatasetting} shows, we consider a high-interest market and a set of maturities ranging from rather short-term American options of 2 months before maturity to long-term American products of 2 years before maturity. Each maturity $T_i$ is associated with a set of strikes $K_i$, $i\in\{1,\dots,5\}$. As for the analysis of De--Ameri\-cani\-za\-tion effects on pricing, we price these options for the five parameter scenarios in Table \ref{Tab_Parameters_Pricing}. Regarding the calibration methodology, we have to make two choices. First we have to decide which option types do we include and second how the objective function looks like.

Regarding the choice of options we first consider only Put options for the whole strike trajectory. Thus, we include in-the-money as well as out-of-the-money options. Second, driven by the fact that the value of out-of-the-money options does not include any intrinsic value and is therefore supposed to reflect the randomness of the market better,%\todo{Reference}
we consider as a second approach to only include out-of-the money puts and out-of-the money calls for the whole set of strikes and maturities. Consequently, in this second study for each $i\in\{1,\dots,5\}$ we consider call option prices for maturities $T_i$ and strikes $k\in K_i$ with $k>1$ and put option prices for maturities $T_i$ and strikes $k\in K_i$ with $k<1$. At-the-money option data, i.e. options with strike $K=1$ is neglected.

Once the American market has been generated, we create an associated second market by applying the De-Americanization routine using the tree model. We thus deamericanize each price individually by calibrating the tree model first and then deriving the associated quasi-European deamericanized price.

Remark~\ref{Remark_Exercise_Region} and Figure~\ref{Toy_Example} described situations in which the De-Americanization routine yields non-unique results. In the calibration to de-Americanized prices we exclude those options that can not be deamericanized uniquely as the following remark underpins.

\begin{remark}[Disregarding non-unique deamericanized prices]
\label{rem:PutOptionsOutinCalib}
As outlined above, we artificially generate American market data for a calibration study on synthetic data. In a first step we calibrate to the generated American prices directly. Here, all generated data is considered. In a second step, we deamericanize the option data and calibrate to the resulting quasi-European options. Here, only those option prices are considered that allow for a unique deamericanized price. Consequently, all American put option prices that violate
	\begin{equation}
	\label{cond:DisregardAtCalib}
		P^\text{put}_{Am}>(K-S_0)^{+}\cdot (1+\delta),\qquad \text{ with } \delta=1 \%,
	\end{equation}
are not de-americanized and thus neglected in the second step.
\end{remark}

The second critical assumption is the objective function. A variety of objective functions is proposed in the literature,e.g. the root mean square error, the average absolute error as a percentage of the mean price, the average absolute error, the average relative percentage error, absolute price differences, relative price differences, absolute implied volatilities, relative implied volatilities (e.g. \cite{detlefsenhaerdle}, \cite{bauer}, \cite{fengler}, \cite{schoutens}).

In the calibration, we take the absolute average squared error (aase) as an objective function and thus minimize
\begin{equation}
\text{aase}=\frac{1}{\#\text{options}}\sum_{\text{option}_k}\vert \text{Market price}_k-\text{Model price}_k\vert^2.\label{objectivefunction}
\end{equation}

The results of the calibration to synthetic data are summarized in Table \ref{Tab_Calibration_Synthetic_Data_Put} for calibrating to put options and in Table \ref{Tab_Calibration_Synthetic_Data_oom} for calibrating to out-of-the-money options.\todo{Note: CEV result not final}

\input{./tex/table_calibration_put}
\input{./tex/table_calibration_oom}
\input{./tex/table_google}
Overall we see that for the CEV model that by calibrating to American options, the parameters more or less match. By calibrating to de-americanized prices however, the volatility parameter $\sigma$ is in most of the cases underestimated and this underestimation is captured by an overestimated $\zeta$ value.

Focusing on the Heston model, we observe that in all calibration to American options the parameters are matched. Comparing calibration results with the according calibration to de--ameri\-cani\-zed data, we clearly see that the three parameters $\gamma$, $\kappa$ and $v_0$ are matched, but the remaining two parameters $\xi$ and $\rho$ show different results. By calibrating to put options, with increasing volatility of volatility parameters $\xi$ the calibrated de--ameri\-cani\-zed parameter overestimates the true parameter. By calibrating to out-of-the-money options, we observe for $\xi$ an underestimation for lower $\xi$ values and an overestimation for higher $\xi$ values. Regarding $\rho$, with increasing volatility of volatility the de--ameri\-cani\-zed parameter tends to underestimate the $\rho$ value. By focusing later on pricing exotic options, we will see whether these two contrary effects will cancel each other or lead to different exotic option prices.\\
For the Merton model we observe the general picture, that by calibrating to American options $\sigma$ is matched. For the other 3 parameters we observe that whenever the jump intensity $\lambda$ is underestimated the according mean $\alpha$ and standard deviation $\beta$ of the jump are adjusted accordingly. Similar observation can be made for calibration to de--ameri\-cani\-zed prices. Here, especially for calibration to out-of-the-money values in $p_4$ and $p_5$ we observe that the $\sigma$ value is additionally not matched.

\subsection{Effects of De--Ameri\-cani\-za\-tion on Calibration to Market Data}
%\label{sec:Calibration_Market}
In order to structure the available data, we follow the methodology applied for the volatility index (VIX) by the Chicago board of exchange (\cite{vix}):
\begin{itemize}
\item Only out-of-the-money put and call options are used
\item The midpoint of the bid-ask spread for each option with strike $K_i$ is considered 
\item Only options with non-zero bid prices are considered
\item Once two puts with consecutive strike prices are found to have zero bid
prices, no puts with lower strikes are considered for inclusion (same for calls)
\end{itemize}
Basically, by this selection procedure, we only select out-of-the-money options that (due to non-zero bid prices) can be considered as liquid. In general, an option price consists of two components reflecting the time value and the intrinsic value of the option. By focusing on out-of-the-money options intrinsic value effects are mostly neglected and the highest option price will be at-the-money. Additionally, the highest market activity is in the at-the-money and slightly out-of-the-money region. 
The calibration results are summarized in Table \ref{Tab_Calibration_Google}\todo{Note: CEV result not final} and illustrated in Figures \ref{Figure_Google_CEV2}, \ref{Figure_Google_Heston2} and \ref{Figure_Google_Merton}. 
\begin{figure}
 \centering 
     \includegraphics[width=\textwidth]{./fig/Google_CEV.jpg}    
     \caption{CEV calibration results of calibrating to Google market data.} 
      \label{Figure_Google_CEV2}
\end{figure}

\begin{figure}
 \centering 
     \includegraphics[width=\textwidth]{./fig/Google_Heston.png}     
     \caption{Heston calibration results of calibrating to Google market data.} 
     \label{Figure_Google_Heston2}
\end{figure}

%\begin{figure}
% \centering 
%    % \includegraphics[width=\textwidth]{./fig/Google_Merton.jpg}
%     \label{Figure_Google_Merton}
%     \caption{Merton calibration results of calibrating to Google market data.} 
%\end{figure}

Here we observe hardly any differences in the parameters. This is most likely due to the low interest rate environment. In this settings, American and European puts coincide and thus, there will hardly be any difference in the prices and thus it is rather normal that we observe similar calibration results.

\subsection{Effects of De--Ameri\-cani\-za\-tion in pricing exotic options}

In the market plain vanilla option prices are traded liquidly and these prices are used to calibrate models. That's what has been done in the previous subsections. But financial institutions are interested in pricing more exotic products like e.g. barrier and lookback options. In this subsection we analyze a down-and-out call option and a lookback option and therewith translate differences in the calibrated models into quantitative prices. The payoff $p(S(T))$ of a down-and-out call option with barrier $B$ is given by
\begin{align}
p(S(T))=(S(T)-K)^{+}\cdot\mathbbm{1}_{\min_{t\le T}S(t)\ge B}. 
\end{align}
For our setting we set $S_0=100$, the barrier $B$ to 90\% of the initial underlying value, $B=0.9\cdot S(0)$ and the strike $K$ to 105\% of the underlying value, $K=1.05S(0)$. For a lookback option we choose the same strike and the payoff $p(S(T))$ is
\begin{align}
p(S(T))=(\bar{S}(T)-K)^{+},\quad with\ \bar{S}(T)=\max_{t\le T}S(t)
\end{align}

And then we priced the exotic options for the parameters in Tables \ref{Tab_Calibration_Synthetic_Data_Put}, \ref{Tab_Calibration_Synthetic_Data_oom} and \ref{Tab_Calibration_Google}. The results are shown in the following Table \ref{Tab_Exotics}.
\input{./tex/table_exotics}
Overall, we observe an different picture through the three models.

In $p_1$ and $p_2$, the scenarios with relatively small volatility we don't see any differences. Thus in case of a small volatility and a medium elasticity of variance $\zeta$ De--Ameri\-cani\-za\-tion seems to work. In the other scenarios we observe that the calibration to de-americanized prices leads to higher exotic option prices if we calibrate to put options only and lower exotic option prices if we calibrate to out-of-the-money options. Thus, the in general lower calibrated $\sigma$ value in combination with an increased $\zeta$ value by calibrating to de-americanized options has this effect in pricing exotic options.

For the Heston model we see that in the cases when the calibration to de-americanized data led to different $\xi$ and $\rho$ values, there are differences in the exotic option prices. More precisely, in all these cases the according barrier and lookback prices are too high. This means that De--Ameri\-cani\-za\-tion causes an systematic overpricing of exotic options.

For the Merton model we see rather small differences for lookback options, but more interestingly, for the down-and-out barrier option we observe differences. This reflects that the different calibrated jump intensity and accordingly adjusted mean and standard deviation of the jumps can buffer De--Ameri\-cani\-za\-tion over the paths when the option can not vanish like in the barrier option case.

Summarizing the results, we see that De--Ameri\-cani\-za\-tion effect matter and can influence the prices of exotic options. Especially, when the assumed model includes jumps. Thus, if available plain vanilla data is of American type, we recommend a direct calibration to American options. However, the computational costs in this case can be an issue. To overcome it, we present a short overview of a model reduction technique, as a reduced basis method (RBM). That is, we substitute the FEM discrete model with the reduced one, which is much cheaper to compute. Then a whole calibration routine is carried out on a reduced system. Of course, the price to pay is the decreased accuracy of the reduced solution compared to the FEM one. However, in the numerical experiments we observe, that these differences have a little influence on the exactness of the calibrated parameter. Several scenarios can be developed with the use of the RBM strategy. For instance, one can start a calibration routine with RBM and later use the calibrated parameter as an initial guess for the calibration process with FEM. In this way, the RBM calibration would lead us relatively fast to the region of local minimum and, hence, the calibration with the FEM afterwards should terminate relatively quickly. 


  

==> tex/preliminaries.tex <==
\section{Introduction}
The most frequently traded single stock options are of American type. In general, there exists a variety of (semi-)closed pricing formulas for European options. For American options, there hardly exist any closed pricing formulas and the pricing under advanced models rely (if possible at all) on heavily demanding numerical techniques.

Hence, this leads to the following approach by practitioners: American option
prices are translated into European prices before the calibration process is
started. This translation is usually done by a simple binomial tree model. This
method is called De--Ameri\-cani\-za\-tion. Figure \ref{DeAm} illustrates the
scheme of this procedure. The motivation behind the De--Ameri\-cani\-za\-tion
method are reduced complexity and lower computational cost. In general, it is
much faster to calibrate to European than American options. In this paper we
quantify the De--Ameri\-cani\-za\-tion error and explore settings in which the
application of the binomial tree to translate American into pseudo-European
options may lead to pitfalls. 
\new{Since the calibration routine is computationally costly and
require many evaluations of the objective for different instances of the
parameters, we also present a model reduction technique, as reduced basis
method, to tackle this difficulty. It allows to reduce significantly the
computational cost of calibrating on American or European options. Different variants of the reduced basis method has been already applied to option pricing~\cite{HSW12b,burkovska,red_bs15} as well as to calibration on option prices, e.g,~\cite{pironneau,pironneau09}. Here we present an application of the reduced basis method~\cite{HSW12b,burkovska} for an efficient calibration process on option prices. Numerical experiments on American option data illustrates the attractiveness of the method in application to option pricing. }
\\
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{./fig/DeAm5.png}
\caption{De--Ameri\-cani\-za\-tion scheme}
\label{DeAm}
\end{center}
\end{figure}
In addition to the usage by practitioners, there is also from theoretical side a connection between American and European put options. Teichmann (2016) \todo{Reference Teichmann 2016, Talk Oberseminar}  states that the value function of an European option coincides with the value function of an American option on the continuation region.  Christensen, Lenga, Kallsen 2015 \todo{reference Christensen, Lenga Kallsen 2015. Mentioned in Teichmann Talk} try to find the cheapest European option dominating a given American option.\\
Our research goal is an detailed analysis of the De--Ameri\-cani\-za\-tion method. We want to exploit what kind of errors are made by the De--Ameri\-cani\-za\-tion method. In the model world we go beyond the Black-Scholes model and explore three different kind of models: The CEV model as local volatility model, the Heston model as stochastic volatility model and the Merton jump diffusion model as jump model. For all these models numerical techniques are available to price American options. First of all we are interested in the question whether the model independently applied binomial tree works for continuous models (CEV and Heston) as well as for models allowing jumps (Merton). Hence American and European puts coincide for zero interest rates we particularly analyze the method in different interest environments and additionally, if the method works more accurately for options with higher or shorter maturities. \\

%Our expectations\footnote{Do we need our expectations here?} are summarized in the following list:
%\begin{itemize}
%\item De--Ameri\-cani\-za\-tion has a stronger effect with increasing maturity
%\item Whereas we expect small differences for the CEV model, we expect more significant differences for the Heston model and assume, that the possibility of jumps may strengthen the gap between European and American style options.
%\end{itemize}
The paper is organized as follows. First, we introduce the binomial tree in
Section 2. Then we briefly describe in Section 3 the models and the pricing
methodology. Section 4 presents the numerical results. Here we first show an
accuracy study before we present De--Ameri\-cani\-za\-tion for solely focussing
on the pricing of options. Afterwards we present calibration result to both,
synthetic data and market data. To conclude the numerical study, effects of
different calibration results in the pricing of exotic options are presented.
In Section 5 we present an overview of the reduced basis method
and together with numerical results demonstrate its efficiency in calibration
to option prices.
Finally, Section 6 concludes the results of this work.


%\subsection{Calibration literature review}

==> tex/pricing.tex <==
\section{Effects of De--Ameri\-cani\-za\-tion on Pricing}
\label{sec:Pricing}

After we have presented our models, we want to firstly focus on differences caused by the De--Ameri\-cani\-za\-tion itself. Therefore, we compare de--americanized American prices with derived European option prices as illustrated in Figure \ref{DeAmPricing} and analyze the differences. 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/DeAmPricing.png}
\caption{First Step De--Ameri\-cani\-za\-tion: Focus on pricing differences}
\label{DeAmPricing}
\end{center}
\end{figure}

The advantage of this approach is that we can purely focus on the De--Ameri\-cani\-za\-tion without mixing it with any calibration issues. In order to do so, we defined the following test set for the range of investigated options. Here we focus on put options due to the fact that non dividend payments lead to the same prices for American and European calls.
\begin{align*}
S_0&=1\\
K&=0.80,0.85,0.90,0.95,1.00,1.05,1.10,1.15,1.20\\
T&=\frac{1}{12},\frac{2}{12},\frac{3}{12},\frac{4}{12},\frac{6}{12},\frac{9}{12},\frac{12}{12},\frac{24}{12}
\end{align*}
First, we describe the observation for each model individually and then in Subsection \ref{subsec:pricing_conclusion} the results are summarized.

\subsection{Pricing differences in the CEV model}
\subsection{Pricing Differences in the Heston Model}
\subsection{Pricing differences in the Merton model}
\subsection{Summary Pricing Differences}
\todo{Maybe results for all 3 models in one block}

==> tex/rbm.tex <==
\section{An Efficient Calibration Process with the Reduced Basis Method}
In order to speed up the computation routine for the calibration algorithm we
employ a reduced basis method (RBM) as an efficient tool for significantly
reducing the computational complexity of solving parametrized PDE's. Since the
methodology of RBM and area of applications are very broad,
our aim here is only to provide brief overview of the method and
its application to options pricing. We refer the interested reader
to, e.g,~\cite{rb_book1,rb_book2,Ha14,buffa,Ha13,grepl2005reduced} and the
references therein, for more details and a theoretical study. 

Consider the discrete problem formulation~\eqref{pr_det} for European options.
For any given parameter $\parmu\in\mathcal{P}$, the cost of fining the solution
depends on the dimension of the discrete approximation space
$\mathcal{N}_V=\dim(V)$ and number of times steps $L$. Obviously for many query
evaluations of the solution at different parameter values,
the computational cost can be extremely high. As a remedy one may employ a model
order reduction, where the space $V$ is approximated by the space $V_N$ of much
lower dimension $N_V\ll\mathcal{N}_V$ and the original model~\eqref{pr_det} is
replaced by a reduced one in $V_N$. There are many model order reduction
techniques in use, attempting to provide such approximation. The idea of the
reduced basis method relies on the parameter dependence of the model and the
construction of the reduced basis space $V_N$ tries to exploit it. In
particular, consider for all $0\leq k\leq L$, a parameter manifold, induced by
the solutions of~\eqref{pr_det} for different parameter values,
\begin{equation}
 \mathcal{M}=\{u^{k}(\parmu)\in V, \quad \parmu\in\mathcal{P}\}\subset
V.
\end{equation}
Then assuming that the manifold admits a sufficient smoothness with respect to
the parameter, we can expect for a given $\parmu\in\mathcal{P}$, to approximate
$u^{k}(\parmu)\in V$ by a linear
combination of only a few elements of $ \mathcal{M}$, called ``snapshots''.
From these snapshots we form the reduced basis $\{\rbv_i\}_{i=1}^{N_V}$ of
$V_N$, $V_N=\spann\{\rbv_i, \quad i=1,\dots, N_V\}\subset V$. 

Given a reduced
basis space $V_N$, the reduced basis approximation of~\eqref{pr_det} reads as
following: For a given $\parmu\in\mathcal{P}$, find $u_N^{k+1}\in V_N$, such
that
\begin{align} 
 \frac{1}{\Delta
t}\left(u_N^{k+1}(\parmu)-u_N^k(\parmu),\phi_N\right)+a(\theta u_N^{k+1}(\parmu)+(1-\theta)u_N^k(\parmu),
\phi_N;\parmu)&=f^ { k+1 } (\phi_N;\parmu), \quad \forall\phi_N\in
V_N.\label{pr_rbm}
 \end{align}
The reduced solution can be represented as $u_N^{k+1}=\sum_{i=1}^{N_V}u_{N
i}^{k+1}\rbv_i$ and the initial condition is given by
$(u_N^0-u^0,v_N)_V=0$. Hence to solve\eqref{pr_rbm} leads to find the
coefficient vector ${\bf u}_N:=[u_{N 1},\dots, u_{N N_V}]\in\mathbb{R}^{N_V}$.
As we can see, the complexity of solving~\eqref{pr_rbm} at each time step $k$,
depends only on the reduced dimension $N_V$. 

The construction of the reduced space $V_N$ and selection of the snapshots, in
general, relies on the greedy strategy. For
time dependent problems, the standard approach is to apply a so called
POD-greedy algorithm~\cite{Ha13}. 

The efficiently of the method is based on an assumption of affine parameter
dependence of
bilinear and linear forms, that is, there exist $\Theta_q^a$,
$\Theta_q^f:\mathcal{P}\rightarrow\mathbb{R}$, such that we can express
$a(\cdot,\cdot;\parmu)=\sum_{q=1}^s\Theta_q^a(\parmu) a^q(\cdot,\cdot)$,
$f(\cdot;\parmu)=\sum_{q=1}^l\Theta_q^f(\parmu) f^q(\cdot)$. Then the
computational routine is decomposed into two stages: the so-called {\it offline}
and {\it online} ones. In the offline routine, which is computationally
expensive, but performed only once, we precompute all parameter independent
quantities. In the online routine, which computationally cheap, performed many
times for every instance of parameter $\parmu\in\mathcal{P}$, we assign all
parameter dependent components and solve the reduced system. The efficiently of
the method is gained via an online routine, which depends on $N_V$ and
independent of the dimension of the original problem $\mathcal{N}_V$.




\subsubsection{Reduced Basis Methods for Variational Inequalities}
Now we extend our consideration to variational inequalities. For more
details we refer to, e.g,~\cite{HSW12,UG13,burkovska}. The reduced basis
solution for American put solves the following reduced basis saddle point
problem. 
\begin{align*}
&\frac{1}{\Delta t}\left(u_N^{k+1}(\parmu)-u_N^k(\parmu),\phi_N\right)+a(
u_N^{k+1}(\parmu),\phi_N;\parmu) -b(\lambda_N^{k+1}(\parmu),\phi_N)  = 
f^{k+1}(\phi_N;\parmu),\\
&b(\eta_N-\lambda_N^{k+1}(\parmu),u_N^{k+1}(\parmu))  \geq
g^{k+1}(\eta_N-\lambda_N^{k+1}(\parmu);\parmu).
\end{align*}
In this case we approximate two solution spaces $V$ and $W$ by $V_N$ and $W_N$
of dimension $\dim(V_N)=N_V\ll\mathcal{N}_N$ and
$\dim(W_N)=N_W\ll\mathcal{N}_W$. The reduced problem reads as follows: For
$\parmu\in\mathcal{P}$ find $u_N^{k+1}(\parmu)\in V_N$ and
$\lambda^{k+1}_N(\parmu)\in M_N$, $0<k\leq L-1$, such that for all $\phi_N\in
V_N$, $\eta_N\in M_N$                  
 
The solutions $u_N^{k+1}(\parmu)$ and $\lambda^{k+1}_N(\parmu)$ are expanded
on the reduced basis of $V_N$ and $W_N$,
$u_N^k(\parmu)=\sum_{i=1}^{N_V}u_{N i}^k(\parmu)\rbv_i$ and
$\lambda_N^k(\parmu)=\sum_{j=1}^{N_W}u_{N j}^k(\parmu)\rbw_i$. These basis
vectors $\rbv_i$, $\rbw_j$, can be generated by e.g., POD-Angle-Greedy
Algorithm~\cite{HSW12b,burkovska}.

We summarize the main ingredients needed for the construction of RBM for
parabolic variational (in-)equalities:
\begin{itemize}
 \item RB spaces $V_N=\spann\{\rbv_i\}_{i=1}^{N_V}$, 
$W_N=\spann\{\rbw_j\}_{j=1}^{N_W}$,  $M_N=\spann_+\{\rbw_j\}_{j=1}^{N_W}$.
 \item RB bases $\rbv_i$, $\rbw_j$, which can be constructed by, e.g, 
POD-(Angle)-Greedy algorithm.
 \item affine parameter dependence \& offline-online decomposition.
\end{itemize}
%-------------------------------------------------------------------
\subsection{Accuracy Study}
For an
approximation of the original problem, we consider the same setting as described before. That is, $\mathcal{N}_V=4753$ and $L=250$. The RB dimension is
chosen as $N_V=200$, $N_W=100$. The accuracy of the reduced basis approximation
with respect to the finite element solution is depicted in
Figure~\ref{fig3} for both European and American options. We can observe the
error difference within $0.1\%$ margin.
\iffalse
The convergence of the RBM w.r.t. different RB dimensions is presented in
Figure~\ref{fig:rb_conv}
\begin{figure}[h!]
\centering
\includegraphics[width=.49\textwidth,height=.23\textheight]
{fig/rbm/basis_error_EO}
 \includegraphics[width=.49\textwidth,height=.23\textheight]
 {fig/rbm/basis_error_AO}
 \caption{RB error convergence in $H^1$-norm for European call (left) and
American put (right).}
 \label{fig:rb_conv}
\end{figure}
\fi

\begin{figure}[h!]
\centering
\includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_EO_10}
 \includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_EO_100}
 \includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_EO_251}\\
\includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_AO_10}
 \includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_AO_100}
 \includegraphics[width=.32\textwidth]{fig/rbm/Sol_scal_difference_AO_251}
 \caption{A scaled error between FEM and RBM solutions for European call (top)
and American put (bottom) at
$t=0.08$ (left), $t=0.8$ (middle) and $t=2$ (right).}
 \label{fig3}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Calibration on Options with RBM}
As a next step we apply the reduced basis method for calibration on American
options. 
As it has been mentioned previously, the many query evaluations of the
solution require a high computation cost. In particular, the calibration
procedure evaluates the objective for many instances of the parameter until the
optimal solution is found. We can observe, that with the use of the reduced
basis method, we can significantly speed up the calculations and obtain the
calibrated parameter within desired accuracy.




\subsubsection{Calibration Results on Synthetic Data Set with RBM}
First, we consider a performance of RBM on a synthetic market data set with
different maturities and strikes. We chose the interest rate $r=0.0198$,
$S_0=590$, maturities $T_i=\frac{1}{12}i$, $i=1,2,3,6,9,12,24$, and the
strikes $K_j=jS_0$, $j=0.5$, $0.55$, $0.6$, $0.65$, $0.7$, $0.75$, $0.8$,
$0.85$, $0.9$, $0.95$, $1$, $1.05$, $1.1$, $1.2$, $1.3$, $1.4$. 
For each pair
$(T_i,K_j)$ we generate the corresponding synthetic data set of European call or
American put options for
the target parameter value $\parmu=( 0.22885,-0.70354,0.072772, 0.72,0.0198, 
0.05)$. 

For $K=1$ and a single input parameter $\mu=(0.2, -0.2, 0.16, 3, 0.0198)$ we
study the runtime performance of RBM in comparison to FEM for both European call
and American put options. The computational time is presented in
Table~\ref{Tablecpu1}. We can observe a significant speed up while computing
already a single trajectory. However, due to an expensive offline cost, it does
not pay off to apply the reduced basis method for a single parameter evaluation. 
\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{FEM solution} & \multirow{2}{*}{RB solution}
& \multicolumn{3}{|c|}{Create Offline data (only once)}\\ \cline{4-6}
                  &                   &                   & snapshots      &   basis    &  reduced data    \\ 
                  \hline\hline
   European    call &    326.7101s               &   0.4549s                & $6.0042\cdot 10^3$s      & $1.0811\cdot 10^5$s      &  $4.5423$s    \\
   \hline
   American put     &   $559.3426$s               &  $2.5925$s                 & $1.2038\cdot 10^5$s      &  $5.5536\cdot 10^4$s     & $3.8676$s \\
   \hline
\end{tabular}\caption{Computational time of using RBM and FEM.}\label{Tablecpu1}
\end{table}

\iffalse
\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{FEM solution} & \multirow{2}{*}{RB solution}
& \multicolumn{3}{|c|}{Create Offline data (only once)}\\ \cline{4-6}
                  &                   &                   & snapshots      &  
basis    &  reduced data    \\ 
                  \hline\hline
   European    call &    326.7101s               &   0.4549s                &
$6.0042\cdot 10^3$s      & $1.0811\cdot 10^5$s      &  $4.5423$s    \\
   \hline
   American put     &   $559.3426$s               &  $2.5925$s                 &
$1.2038\cdot 10^5$s      &  $5.5536\cdot 10^4$s     & $3.8676$s \\
   \hline
\end{tabular}\caption{Computational time for RBM and FEM
solvers}\label{Tablecpu1}
\end{table}
\fi
Next, we perform the calibration routine with synthetic data set using both
FEM and RBM. The corresponding results are plotted in Figure~\ref{fig4}. The
calibrated parameter using RBM, $\parmu=(0.29959,-0.68997,0.064429,
1.8246,0.0198, 0.047484)$, is close to the one, obtained using FEM, 
$\parmu=(0.22885,-0.70354,0.072772, 0.72,0.0198, 0.05)$ apart from the parameter $\kappa$. This is due to a fact, that in practice, it is often observable, that a parameter $\kappa$ is not price sensitive. From the run-time performance, we can observe that RBM is 50 times faster than FEM. 

\begin{figure}[ht!]
\centering
\includegraphics[width=.48\textwidth]{fig/rbm/09Feb15_simulated_data_3_AO_put_119_putput_RBM0_lsq_surf}
\includegraphics[width=.48\textwidth]{fig/rbm/09Feb15_simulated_data_3_AO_put_119_putput_RBM1_lsq_surf}
 \caption{Calibrated and market data with FEM (right) and RBM (left). The computational time with FEM is $14,74$ hours and with RBM is 17.33 min.}
 \label{fig4}
\end{figure}


\iffalse
\begin{figure}[ht!]
\centering
\includegraphics[width=.49\textwidth]{fig/rbm/09Feb15_simulated_data_3_AO_put_119_putput_RBM0_lsq_surf_dif}
\includegraphics[width=.49\textwidth]{fig/rbm/09Feb15_simulated_data_3_AO_put_119_putput_RBM1_lsq_surf_dif}
 \caption{An error surface between calibrated and market data using FEM solver (left) and RBM (right).}
 \label{fig6}
\end{figure}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Calibration Results on Google Options with RBM}
Next, we present calibration results for a market data. Namely, consider the OTM Google option data with $S_0=523.755$ on
$t_0=02.02.2015$, consisting of 206 American put options. The results are presented in
Figure~\ref{fig:google_rb}. Similarly as for the synthetic data set, we can
observe a good fit to the market data using both the FEM and RBM. 
The efficient performance of the RBM in comparison to FEM is also demonstrated.
In contrast, for this data set the exact solution is not known, we can only
observe that the values of the calibrated parameters, obtained using FEM and RBM
does not deviate too much. They are given as follows:
$\parmu=(0.9,-0.29923,0.067399,
3.0397,0.0198, 0.54838)$ (FEM) and $\parmu=(0.89999,-0.29235,0.06929,
3.1158,0.0198, 0.052815)$ (RBM).
\begin{figure}[ht!]
\centering
\includegraphics[width=.49\textwidth]{fig/rbm/28Feb15_GoogleData_2015_processed_all_maturities_putput_RBM0_lsq_surf}
\includegraphics[width=.49\textwidth]{fig/rbm/28Feb15_GoogleData_2015_processed_all_maturities_putput_RBM1_lsq_surf}
 \caption{Calibrated and market data with FEM (right) and RBM (left). The computational time with FEM is $>10$ hours and with RBM is 58 min.}
 \label{fig:google_rb}
\end{figure}

From the results of this section, we can conclude, that the RBM can
be efficiently applied to calibrate on American options to gain a significant
speed up of the calibration routine. Hence, one can use it as an alternative
mean for the De-Americanization procedure by directly calibrating to American
options instead of the De-Americanized one. \todo{discuss in which perspective to put a conclusion}



==> tex/results.tex <==
\section{Effects of De--Ameri\-cani\-za\-tion on Pricing}
\label{sec:Pricing}

After we have presented our models, we want to firstly focus on differences caused by the De--Ameri\-cani\-za\-tion itself. Therefore, we compare de--americanized American prices with derived European option prices as illustrated in Figure \ref{DeAmPricing} and analyze the differences. 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/DeAmPricing.png}
\caption{First Step De--Ameri\-cani\-za\-tion: Focus on pricing differences}
\label{DeAmPricing}
\end{center}
\end{figure}

The advantage of this approach is that we can purely focus on the De--Ameri\-cani\-za\-tion without mixing it with any calibration issues. In order to do so, we defined the following test set for the range of investigated options. Here we focus on put options due to the fact that non dividend payments lead to the same prices for American and European calls.
\begin{align*}
S_0&=100\\
K&=80,85,90,95,100,105,110,115,120\\
T&=\frac{1}{12},\frac{2}{12},\frac{3}{12},\frac{4}{12},\frac{6}{12},\frac{9}{12},\frac{12}{12},\frac{24}{12}
\end{align*}
First, we describe the observation for each model individually and then in Subsection \ref{subsec:pricing_conclusion} the results are summarized.\\
\textbf{\color{blue}{@ Wim: Here we investigated two interest rate settings: 0\% and 7\%. Do you think this is enough or do you suggest other scenarios to take a look at?}}

\subsection{Pricing differences in the CEV model}
For the CEV model we defined a set of scenarios as illustrated in Table \ref{ScenCEV}. Overall, we investigated 8 different parameter settings with a low, a moderate and a relatively high value for the parameter $\sigma$ and relatively high values for the parameter $\rho$. Note that $\rho=1$ reflects the Black Scholes model (\cite{blackscholes}). Additionally, each of this 8 parameter settings is investigated for an interest rate of zero and for a very high interest rate of $r=7\%$. Table \ref{ScenCEV} summarizes each scenario including the average pricing difference over 72 prices (9 strikes and 8 maturities) and the maximum pricing error. Additionally, we see in Figures \ref{Results_CEV_1} and \ref{Results_CEV_2} an illustration of the option prices and the pricing differences in each scenario.\\
By taking a look at the results we observe that for every parameter combination for an interest rate of $r=0\%$ the average difference and the maximum error are significantly smaller than in the case $r=7\%$. More specifically, in the $r=0\%$ case the pricing differences are close to zero. This observation is supported by the fact, that for zero interest rates American and European puts coincide which can easily be shown by applying Jensen's inequality.  Thus, in a zero interest rate setting there is only a very small De--Ameri\-cani\-za\-tion effect.

By focusing on the results for an interest rate of $7\%$, we clearly observe pricing differences and thus, De--Ameri\-cani\-za\-tion effects. In general, we observe higher differences in the in-the-money region (Strike $K>100$). In Scenarios 6, 12 and 18 the highest maximum errors are observed. In this three scenarios the volatility factor $\sigma$ is set to a low value of $0.1$. Therefore, the volatility is scaled to a relatively low level and it becomes advantageous to early exercise the put options.
At this point we have to understand the differences in American and European put prices first in order to understand differences resulting from the De--Ameri\-cani\-za\-tion methodology applying the binomial tree. For American options we generally observe that the option prices increase with increasing maturity, because an increased maturity allows the investor to possibly exercise in a broader time band, but the shorter maturity time band is still completely covered. For European options we have a more diverse picture depending on the parameters of the model as well as the interest rate. Especially by looking at the option price surface illustrated in Figures \ref{Results_CEV_1} and \ref{Results_CEV_2}, we observe that for $r=0\%$ the option price surface exceeds the value of 20 in any scenario, whereas for $r=7\%$ the option prices are bounded by 20 except in the scenario 16. Furthermore, for an interest rate of $r=0\%$ the option price surface is smoothly increasing with increasing maturity, whereas for $r=7\%$ the option price surface generally decreases over time (scenarios 2, 4, 6, 8, 10, 12 and 18), but for scenarios 14 and 16 the option price surface remains relatively stable. Here it is interesting, that only in the Black Scholes ($\rho=1$) scenarios  14 and 16 the option prices do not decline over time, whereas for all other scenarios including the Black Scholes related scenario 18 (this one has a very low volatility value $\sigma=0.1$) the option price for in-the-money options decreases over time. \\
Here we have to reflect, that in the case of interest rate $r=7\%$ our underlying asset has a high positive drift of exactly $7\%$ and therefore, the underlying value will increase over time, especially when the diffusion part plays only a minor role in the evolution of the underlying. And of course, when the underlying value is drift dominated, it increases and thus, the put prices decrease. On the other hand in the $r=0\%$ case the development is only driven by the diffusion component and due to the characteristics of the local volatility in the CEV model, i.e. increasing volatility if the underlying value is decreasing resp. decreasing volatility if the underlying value is increasing, we observe a tendency towards declining underlying values over time and therefore, the put option prices increase. In the Black Scholes related scenarios ($\rho=1$) of course the volatility is symmetric and therefore, we observe relatively stable option prices.\\
As a second step in our analysis we want to focus on in which maturity and strike regions the highest pricing differences occur. Naturally, the pricing differences are higher in the in-the-money region, but on the one hand we observe scenarios, in which the pricing difference only occur in the in-the-money region, namely scenarios 2, 5, 6, 7, 8, 10, 12, 17, 18, whereas in the other scenarios also pricing differences occur in the out-of-the-money region and at-the-money. 
 




\subsection{Pricing Differences in the Heston Model}
The results for the Heston model are illustrated in Table \ref{ScenHeston}. Analogue to the CEV model the average pricing difference over 72 prices and the maximum pricing error are shown for each scenario. Due to the fact that the Heston model incorporates more model parameters, the number of investigated scenarios increased to 26 scenarios, containing 13 parameter combinations, each for zero interest rates and for an interest rate of $r=7\%$. Figures \ref{Results_Heston_1}, \ref{Results_Heston_2} and \ref{Results_Heston_3} illustrate the pricing differences in each scenario as well as the option prices. The first observation is similar to the CEV case: For zero interest rates the pricing differences are rather small, whereas for high interest rates $r=7\%$ the pricing differences are significantly higher.  Additionally, also for the Heston model we observe that the pricing differences and thus, the De--Ameri\-cani\-za\-tion effects increase with increasing maturities and increasing strikes. But overall, in cases of $r=7\%$ the pricing differences are significantly higher than in the corresponding zero interest rate case, although the absolute errors are lower compared to the CEV case. This may be explained due to the fact, that the incorporated stochastic volatility influences the SDE of the underlying more symmetrically. Analogously to the CEV model this pricing exercise has shown, that the approach in the data selection of only including out-of-the-money options may cause lower De--Ameri\-cani\-za\-tion effects, but that for the Heston model choosing out-of-the-money options in the calibration is no guarantee that the De--Ameri\-cani\-za\-tion methodology may not lead to different calibrated model parameters.



\subsection{Pricing differences in the CGMY model}

\subsection{Summary Pricing Differences}
\label{subsec:pricing_conclusion}
In this subsection we summarize the results from the analysis of the De--Ameri\-cani\-za\-tion effects regarding the pricing. 
So far, for the CEV and Heston models we have seen that the interest rate is one driver of the De--Ameri\-cani\-za\-tion effect. In high interest rate settings American and European puts differ significantly and therefore the binomial tree translations of American prices do not coincide with the European prices. Our second observation has been that the pricing differences increase with increasing maturity and occur significantly higher in the in-the-money region. For the CEV model we observe stronger effects with asymmetric volatility ($\rho<< 1$) and for the Heston model with higher correlation $\rho$ and higher volatility of volatility $\zeta$.
Thus, our results suggest to select in the calibration only out-of-the-money options because these may cause lower De--Ameri\-cani\-za\-tion effects. However,already this pricing exercise has shown, that for the CEV and the Heston models choosing out-of-the-money options in the calibration is no guarantee that the De--Ameri\-cani\-za\-tion methodology may not lead to different calibrated model parameters. Especially in high interest rate environments we expect different calibration results if we compare a direct calibration to American options with a calibration to De--Ameri\-cani\-zed data.\\
\textbf{\color{blue}{@ Wim: Here we say that by looking at oom options, the De--Ameri\-cani\-za\-tion effect will be smaller and thus, it could be beneficial to consider oom options in the calibration. Could it be possible, that the De--Ameri\-cani\-za\-tion effect is just not so visible. What do you think of doing the following experiment in the calibration: 1) Select only oom option and investigate the effect for exotic options. 2) Select only itm options in the calibration and investigate the effect? }}







==> tex/results_calibration.tex <==
\section{Effects of De--Ameri\-cani\-za\-tion on Calibration}	

After we have investigated De--Ameri\-cani\-za\-tion effects in the pricing we present in this section the calibration results to the Google market data described in Section \ref{calibration_methodology}. 

\subsection{CEV model}
The calibration results to the Google market data (Table \ref{GoogleDaten}) are illustrated in Figure \ref{CEV_Google}. Following the De--Ameri\-cani\-za\-tion methodology described in Figure \ref{DeAm}, Figure \ref{CEV_Google_cali} shows the calibration results to the De--Ameri\-cani\-zed Google market data. Finally, Table \ref{CEV_Google_Table} illustrates the differences in the calibrated model parameters.\\
Overall, our data selection criteria described in Section \ref{calibration_methodology} has lead to a pool of 480 options. With only two parameters within the CEV model, we are pleased with our calibration results to the American data. The calibrated parameters only differ slightly. However, the pricing exercise in Section \ref{sec:Pricing} allows us to explain the results with the relatively low interest rate environment. As an additional step we will create synthetic data in a high interest rate ($r=7\%$) and look at the calibration results in this setting. To create the synthetic data, we stay in the framework and price the options from Table \ref{GoogleDaten} for an arbitrary parameter set and with $r=7\%$. Table \ref{CEV_Syn_Data_Table} shows the calibration results in this setting. Here, the calibrated parameters differ slightly stronger than in for the Google market data. So far, we have seen stronger parameter differences if the interest rate is higher. In Subsection \ref{subsec:Effects_For_Exotics} the consequences of different calibration results for exotic options are investigated.

\begin{table}[h]
\begin{center}
 \begin{tabular}{|c|c|c|c|}
 	\hline
  Calibrated to&$\sigma$&$\rho$&ape\\
  \hline
  American data&0.25000&0.9783&3.0\\
  \hline
  De--Ameri\-cani\-zed data&0.2500&0.9784&3.2\\
  \hline
 \end{tabular}
 \caption{CEV model: Comparison of calibration results for Google market data following De--Ameri\-cani\-za\-tion methodology methodology}
 \label{CEV_Google_Table}
 \end{center}
\end{table} 

\begin{table}[h]
\begin{center}
 \begin{tabular}{|c|c|c|c|}
 	\hline
  Calibrated to&$\sigma$&$\rho$&ape\\
  \hline
  American data&0.25&0.9789&0.18\\
  \hline
  De--Ameri\-cani\-zed data&0.25&0.9784&3.2\\
  \hline
 \end{tabular}
 \caption{CEV model: Comparison of calibration results for synthetic data following De--Ameri\-cani\-za\-tion methodology methodology. The synthetic data was created for $\sigma=0.25,\ \rho=0.98$}
 \label{CEV_Syn_Data_Table}
 \end{center}
\end{table} 


\subsection{Heston model}
Figure \ref{Heston_Google_cali} shows the calibration results of the Heston model to the Google market data. Finally, Table \ref{Heston_Google_Table} summarizes the two calibration results. Similarly to the results of the CEV model we only observe slightly differences in the option parameters. Analogously to the previous subsection we created synthetic data and Table \ref{Heston_Syn_Data_Table} summarizes the results. Here we see that the parameter differences are in a similar range than the different parameters via a calibration to Google market data. Subsection \ref{subsec:Effects_For_Exotics} analyzes the consequences of different calibration results for exotic options.


\begin{table}[h]
\begin{center}
 \begin{tabular}{|c|c|c|c|c|c|c|}
 	\hline
  Calibrated to&$\zeta$&$\rho$&$\theta$&$\kappa$&$v_0$&ape\\
  \hline
  American data&0.22876&-0.68582&0.058463&4.3095&0.065061&0.9\\
  \hline
  De--Ameri\-cani\-zed data&0.22474&-0.69374&0.058638&4.148&0.064657&0.8\\
  \hline
 \end{tabular}
 \caption{Heston model: Comparison of calibration results for Google market data following De--Ameri\-cani\-za\-tion methodology methodology}
 \label{Heston_Google_Table}
 \end{center}
\end{table}
\begin{table}[h]
\begin{center}
 \begin{tabular}{|c|c|c|c|c|c|c|}
 	\hline
  Calibrated to&$\zeta$&$\rho$&$\theta$&$\kappa$&$v_0$&ape\\
  \hline
  American data&0.4&-0.8&0.16&3.5&0.15&$5.7\cdot10^{-10}$\\
  \hline
  De--Ameri\-cani\-zed data&0.40108&-0.080473&0.16187&3.4412&0.14844&0.007\\
  \hline
 \end{tabular}
 \caption{Heston model: Comparison of calibration results for Google market data following De--Ameri\-cani\-za\-tion methodology methodology. The synthetic data was created for $\zeta=0.4,\ \rho=-0.8,\ \theta=0.16,\ \kappa=3.5,\ v_0=0.15$}
 \label{Heston_Syn_Data_Table}
 \end{center}
\end{table}

\subsection{CGMY model}

\subsection{Impacts for Option Valuation and Risk Management}
\label{subsec:Effects_For_Exotics}
The previous subsections have shown differences in the calibration results resulting from the De--Ameri\-cani\-za\-tion methodology for all three models. Naturally, in practice the plain vanilla call and put options are used \footnote{Source?} are used to calibrate the model and then e.g. banks are able to price with the calibrated model parameters more exotic options. In this section we will illustrate the impact of differences in the calibrated parameters within this context.

\textbf{\color{blue}{@ Wim: Which exotic options do we choose in order to question pricing differences resulting from different parameters?}}

Embedded in the field of model and parameter risk \footnote{literature} practitioners should be careful opening the third box De--Ameri\-cani\-za\-tion additionally without being aware of the incorporated risks. Especially in Section \ref{PricingDifferences} we have illustrated scenarios in which one may expect strong De--Ameri\-cani\-za\-tion effects. 
\input{./tex/rbm}
\section{Conclusion}



==> tex/roadmap.tex <==
\section{Status quo}
\begin{itemize}
\item CEV model: Code (FEM) fixed and ready
\item Heston: Code (FEM) ready
\item CGMY model: Code (FEM) ready
\end{itemize}
\section{Next steps}
\begin{enumerate}
\item Pricing of American and European options for various parameters and then focus on De--Ameri\-cani\-za\-tion effect.
\item Calibration to created model data
\item Calibration to market data 
\end{enumerate}
\section*{1-Pricing of American and European options for various parameters and then focus on De--Ameri\-cani\-za\-tion effect}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/DeAmPricing.png}
\caption{First Step De--Ameri\-cani\-za\-tion: Focus on pricing differences}
\label{DeAm}
\end{center}
\end{figure}
\begin{itemize}
\item Focus on differences caused by the De--Ameri\-cani\-za\-tion itself. I.e. comparing de--americanized American prices with derived European option prices (as discussed with Wim Schoutens)
\item Not mixing "De--Ameri\-cani\-za\-tion effect" and calibration errors
\item Get a feeling for the parameter sensitivities
\item Set of put options:\\
\begin{align*}
S_0&=100\\
K&=80,85,90,95,100,105,110,115,120\\
T&=\frac{1}{12},\frac{2}{12},\frac{3}{12},\frac{4}{12},\frac{6}{12},\frac{9}{12},\frac{12}{12},\frac{24}{12}
\end{align*}
\item Model parameters as well as interest rate $r$ vary.
\end{itemize}
\newpage
\section*{2-Calibration to created model data and 3-Calibration to market data}
\begin{itemize}
\item First calibration to created "model data" to get a feeling for the calibration error?
\item Objective function calibration
\begin{align*}
arpe=\frac{1}{number\ of\ options}\sum_{options}\frac{\vert Market\ price-Model\ price\vert}{Market\ price}
\end{align*}
\item Issue market data: Which selection procedure should we do?
\item Methodology applied for the volatility index (VIX) by the Chigaco board of exchange (\cite{vix}):
\begin{itemize}
\item Only out-of-the money put and call options are used
\item The midpoint of the bid-ask spread for each option with strike $K_i$ is considered 
\item Only options with non-zero bid prices are considered
\item Once two puts with consecutive strike prices are found to have zero bid
prices, no puts with lower strikes are considered for inclusion (same for calls)
\end{itemize}
\end{itemize}

==> tex/table_calibration_heston.tex <==
\begin{table}[]
\centering
\begin{tabular}{cl|cccccc}
                              \multicolumn{8}{c}{Calibration to only put options}                                                     \\
                             &      & $\xi$           &$\rho$          & $\gamma$           & $\kappa$          & $v_0$           & aase       \\

\multirow{3}{*}{$p_1$		} & true   &  0.1     & -0.2   &  0.07     &  0.1    &  0.07    &  ---    \\
                             & Am &    0.1002   &-0.1999     &0.07       & 0.1026    &0.07      & 1.43e-13    \\ 
                             & DeAm &   0.1    & -0.4839    &   0.0651    &  0.5144    &  0.0695   &  1.50e-7    \\                             
                             \hline
\multirow{3}{*}{$p_2$		} & true   & 0.25      &  -0.5  &  0.1     & 0.4     &  0.1    & ---     \\
                             & Am &   0.25    &   -0.5  &    0.1   &      0.4 &    0.1  & 6.47e-23    \\ 
                             & DeAm &     0.2667  &   -0.5067  &   0.0978    &0.4374      &   0.0992  &  3.28e-8    \\                             
                             \hline
\multirow{3}{*}{$p_3$		} & true   &  0.4     & -0.5   &  0.15     &   0.6   & 0.15     &  ---    \\
                             & Am &     0.4  &    -0.5 &       0.15&  0.6   &     0.15 &  7.15e-16   \\ 
                             & DeAm &      0.4684 &  -0.437   &    0.1544   &    0.6806  & 0.1495    &  6.04e-9    \\                             
                             \hline
\multirow{3}{*}{$p_4$		} & true   &   0.55  	  & -0.45   &  0.2     &  1.2    &  0.2    &  ---    \\
                             & Am &      0.55 		&    -0.45 &      0.2 &    1.2 &    0.2  &   1.44e-17  \\ 
                             & DeAm &       0.5773	&     -0.4298&      0.2046 &  1.1975    &  0.1986   &  2.86e-9    \\                             
                             \hline                                        
\multirow{3}{*}{$p_5$		} & true   	& 0.7      &  -0.8  &    0.3   &   1.4   & 0.3     & ---     \\
                             & Am 		&    0.7   &     -0.8&   0.3    &  1.4   &   0.3   &  1.68e-17   \\ 
                             & DeAm 	&      0.8504 &  -0.7057   &  0.3136     &  1.5832    & 0.2993    &  1.31e-8    \\                             
                             \hline
                             \\
                            \multicolumn{8}{c}{Calibration to out-of-the-money options}                                                     \\

                             &      & $\xi$           &$\rho$          & $\gamma$           & $\kappa$          & $v_0$           & aase       \\
\multirow{3}{*}{$p_1$		} & true   	& 0.1      & -0.2   &   0.07    &  0.1    & 0.07     &  ---    \\
                             & Am 		&    0.1006   &  -0.1987   & 0.07      & 0.1049    & 0.07     & 4.73e-13    \\ 
                             & DeAm 	&     0.1  &  -0.1949   &   0.0665    & 0.2292     &  0.07   & 1.32e-8     \\                             
                             \hline
\multirow{3}{*}{$p_2$		} & true   	& 0.25      & -0.5   & 0.1      & 0.4     & 0.1     & ---     \\
                             & Am 		& 0.25      & -0.5    &   0.1    &   0.4  &   0.1   &  2.99e-17   \\ 
                             & DeAm 	&  0.2199     &  -0.5   &    0.0885   & 0.1618     & 0.1    &   5.76e-9   \\                             
                             \hline
\multirow{3}{*}{$p_3$		} & true   &0.4       & -0.5   &    0.15   &   0.6   & 0.15     & ---     \\
                             & Am 		&  0.4     &   -0.5  &   0.15    &    0.6 &    0.15  &7.03e-18    \\ 
                             & DeAm 	&     0.3970  &   -0.5  &    0.1517   &  0.5413    &0.1494     &4.68e-9      \\                             
                             \hline
\multirow{3}{*}{$p_4$		} & true   & 0.55      &  -0.45  & 0.2      &   1.2   &  0.2    &  ---    \\
                             & Am 		&    0.55   & -0.45    &  0.2     &   1.2  &  0.2    &  8.41e-22   \\ 
                             & DeAm 	&    0.5625   &  -0.4369   &  0.2035     & 1.2198     &  0.1988   & 4.50e-9     \\                             
                             \hline
\multirow{3}{*}{$p_5$		} & true   & 0.7      & -0.8   &   0.3    &  1.4    &  0.3    & ---     \\
                             & Am 		&   0.7    &  -0.8   &    0.3   &   1.4  & 0.3     &  8.58e-23   \\ 
                             & DeAm 	&   0.7763    &  -0.7602   & 0.3073      &1.7021      & 0.2979    & 2.34e-8     \\                             
                             \hline
\end{tabular}
\caption{Calibration results for calibrating to put options only and out-of-the-money options.}
\label{Tab_Calibration_Heston}
\end{table}



==> tex/table_calibration_merton.tex <==
\begin{table}[]
\centering
\begin{tabular}{cl|ccccc}
                            \multicolumn{7}{c}{Calibration to only put options}                                                     \\
                             &      & $\sigma$           &$\alpha$          & $\beta$           & $\lambda$                    & aase       \\

\multirow{3}{*}{$p_1$		} & true   &  0.20     &  -0.01  & 0.01      &  1    &  ---          \\
                             & Am &   0.20    &  0.01   &    0.05   &   0.29  &    1.07e-10       \\ 
                             & DeAm &   0.20    &  -0.06   & 0.03      &  0.37    &8.37e-8           \\                             
                             \hline
\multirow{3}{*}{$p_1$		} & true   & 0.15      &-0.05    & 0.05      &2      & ---           \\
                             & Am &    0.15   &   -0.06  &   0.05    &   1.55  &  2.69e-11         \\ 
                             & DeAm &  0.14     &   -0.10  &  0.01     &  1.31    & 1.63e-7          \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   & 0.20  &-0.10    &0.10       &3      &        ---    \\
                             & Am &     0.22  & -0.19    &    0.07   & 1.31    &         8.83e-10  \\ 
                             & DeAm &   0.16    & -0.05    &      0.11 &   5.04   &    3.12e-8       \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   &0.10       &-0.10    & 0.20      &5      &  ---          \\
                             & Am &     0.10  &   -0.10  &    0.20   &   5.00  &    1.22e-13       \\ 
                             & DeAm &    0.09   & -0.09    &  0.21     &    4.90  &      2.19e-7     \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   &0.10  &-0.15    &0.20       & 7     &  ---          \\
                             & Am &    0.10   & -0.15    &   0.20    & 7.00    & 8.96e-13          \\ 
                             & DeAm &   0.05    & -0.11    &    0.21   &   7.95   &   1.73e-7        \\                             
                             \hline
                             \\
                             \multicolumn{7}{c}{Calibration to out-of-the-money options}                                                                                 \\
                             &      & $\sigma$           &$\alpha$          & $\beta$           & $\lambda$                    & aase       \\
\multirow{3}{*}{$p_1$		} & true   & 0.20      &-0.01    &0.01       & 1     & ---            \\
                             & Am &   0.20    &   0.00  &   0.05    &   0.32  &   1.35e-10        \\ 
                             & DeAm &     0.20  &  -0.02   &  0.04     &0.30      &     3.80e-9      \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   & 0.15      &-0.05    & 0.05      &2      &  ---          \\
                             & Am 		&   0.16    & -0.10    & 0.04      &  0.66   & 1.91e-10          \\ 
                             & DeAm 	&  0.15     & -0.11    &  0.03     & 0.74     &   2.22e-8        \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   & 0.20      & -0.10   & 0.10      & 3     &    ---        \\
                             & Am 		&    0.22   & -0.19    &   0.07    &1.32     & 5.47e-10          \\ 
                             & DeAm 	&    0.19   &  -0.17   &  0.09     &    1.88  &   3.33e-7        \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   & 0.10      & -0.10   &  0.20     &  5    &  ---          \\
                             & Am 		& 0.10      & -0.10    & 0.20      & 5.00    &  6.29e-16         \\ 
                             & DeAm 	&  0.15     &  -0.14   &  0.22     &  3.63    &     6.53e-7      \\                             
                             \hline                             
\multirow{3}{*}{$p_1$		} & true   & 0.10      & -0.15   & 0.20      &  7    &   ---         \\
                             & Am 		& 0.10      & -0.15    &   0.20    & 7.00    & 5.00e-13          \\ 
                             & DeAm 	&  0.05     &  -0.20   &       0.23&   5.08   &      1.67e-6     \\                             
                             \hline           
\end{tabular}
\caption{Calibration results for calibrating to put options only and out-of-the-money options. Due to the effect of non-unique De-Americanization results, some option prices have been neglected in the calibration to De-Americanized option data, as Remark~\ref{rem:PutOptionsOutinCalib} explains. In scenarios  $p_1$ and $p_2$ of the Merton model, 5 prices have been excluded in the calibration to only put options.}
\label{Tab_Calibration_Merton}
\end{table}


==> tex/table_calibration_merton_v2.tex <==
\begin{table}[h!]
\centering                                                                                                       
\begin{tabular}{ccl|ccccc}
 &\multicolumn{7}{c}{Merton}  \\
                                                   &                                                 &      & $\sigma$           &$\alpha$          & $\beta$           & $\lambda$                    & aase \\
\multirow{5}{*}{$p_1$}                             &                                                 & true &  0.20     &  -0.01  & 0.01      &  1    &  ---          \\
                                                   & \multirow{2}{*}{Put}                            & Am   &  0.20    &  0.01   &    0.05   &   0.29  &    1.07e-10                     \\
                                                   &                                                 & DeAm &  0.20    &  -0.06   & 0.03      &  0.37    &8.37e-8                      \\
                                                   & \multirow{2}{*}{oom}                            & Am   &  0.20    &   0.00  &   0.05    &   0.32  &   1.35e-10                            \\
                                                   &                                                 & DeAm &   0.20  &  -0.02   &  0.04     &0.30      &     3.80e-9                    \\
												   \hline
\multirow{5}{*}{$p_2$}                             &                                                 & true &   0.15      &-0.05    & 0.05      &2      & ---   \\
                                                   & \multirow{2}{*}{Put}                            & Am   &   0.15   &   -0.06  &   0.05    &   1.55  &  2.69e-11      \\
                                                   &                                                 & DeAm &     0.14     &   -0.10  &  0.01     &  1.31    & 1.63e-7             \\
                                                   & \multirow{2}{*}{oom}                            & Am   &    0.16    & -0.10    & 0.04      &  0.66   & 1.91e-10                    \\
                                                   &                                                 & DeAm &    0.15     & -0.11    &  0.03     & 0.74     &   2.22e-8             \\
												   \hline
\multirow{5}{*}{$p_3$}                             &                                                 & true &   0.20  &-0.10    &0.10       &3      &        ---       \\
                                                   & \multirow{2}{*}{Put}                            & Am   &    0.22  & -0.19    &    0.07   & 1.31    &         8.83e-10            \\
                                                   &                                                 & DeAm &     0.16    & -0.05    &      0.11 &   5.04   &    3.12e-8        \\
                                                   & \multirow{2}{*}{oom}                            & Am   &     0.22   & -0.19    &   0.07    &1.32     & 5.47e-10           \\
                                                   &                                                 & DeAm &      0.19   &  -0.17   &  0.09     &    1.88  &   3.33e-7              \\
												   \hline
\multirow{5}{*}{$p_4$}                             &                                                 & true &  0.10       &-0.10    & 0.20      &5      &  ---        \\
                                                   & \multirow{2}{*}{Put}                            & Am   &    0.10  &   -0.10  &    0.20   &   5.00  &    1.22e-13             \\
                                                   &                                                 & DeAm &   0.10      & -0.10    & 0.20      & 5.00    &  6.29e-16          \\
                                                   & \multirow{2}{*}{oom}                            & Am   &   0.09   & -0.09    &  0.21     &    4.90  &      2.19e-7     \\
                                                   &                                                 & DeAm &   0.15     &  -0.14   &  0.22     &  3.63    &     6.53e-7                \\
												   \hline
\multirow{5}{*}{$p_5$}                             &                                                 & true &  0.10  &-0.15    &0.20       & 7     &  ---        \\
                                                   & \multirow{2}{*}{Put}                            & Am   &   0.10   & -0.15    &   0.20    & 7.00    & 8.96e-13                \\
                                                   &                                                 & DeAm &   0.05    & -0.11    &    0.21   &   7.95   &   1.73e-7             \\
                                                   & \multirow{2}{*}{oom}                            & Am   &  0.10      & -0.15    &   0.20    & 7.00    & 5.00e-13                \\
                                                   &                                                 & DeAm &   0.05     &  -0.20   &       0.23&   5.08   &      1.67e-6           \\
												   \hline                      
\end{tabular}
\caption{Calibration results for calibrating to put options only and out-of-the-money options. Due to the effect of non-unique De-Americanization results, some option prices have been neglected in the calibration to De-Americanized option data, as Remark~\ref{rem:PutOptionsOutinCalib} explains. In scenarios  $p_1$ and $p_2$ of the Merton model, 5 prices have been excluded in the calibration to only put options.}
\label{Tab_Calibration_Merton}
\end{table}

==> tex/table_calibration_oom.tex <==
\begin{sidewaystable}[]
\centering
\small
\begin{tabular}{cl|lll|llllll|lllll}
                       &      & \multicolumn{3}{c|}{CEV}                                       & \multicolumn{6}{c|}{Heston}                                                                                                                              & \multicolumn{5}{c}{Merton}                                                                          \\
                       &      & \multicolumn{1}{c}{$\sigma$} & \multicolumn{1}{c}{$\xi$} & aase & \multicolumn{1}{c}{$\zeta$} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{$\gamma$} & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{$v_0$} & aase & \multicolumn{1}{c}{$\sigma$} & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{$\beta$} & \multicolumn{1}{c}{$\lambda$} & aase \\
\hline
\multirow{3}{*}{$p_1$} & true & \multicolumn{1}{c}{0.2}         & \multicolumn{1}{c}{0.5}      &  -   & 0.1& -0.2&0.07 & 0.1& 0.07& --   & 0.20  & -0.01  & 0.01  & 1  &  -   \\
                       & Am   &                 0.1997             &     0.4996                      &   4.52e-6  &     0.1006                        & -0.1987                           &                             0.07 &             0.1049                 & 0.07                          & 4.73 e-13   &               0.20        &                       0.00 &     0.05   &                      0.32 &    1.35e-10 \\
                       & DeAm &               0.1793               &       0.9609                    &   2.75e-4  &    0.1                         &  -0.1949                          &0.0665                              &0.2292                              &    0.07                       &  1.32e-8   &  0.20  &   -0.02    &  0.04 & 0.30  & 3.80e-9 \\
\hline
\multirow{3}{*}{$p_2$} & true & \multicolumn{1}{c}{0.275}         & \multicolumn{1}{c}{0.6}      &    - & 0.25&-0.5&0.1&0.4&0.1& --    & 0.15  & -0.05  & 0.05  & 2  &   -  \\
                       & Am   &             0.2736                 &       0.5978                    &   1.91e-6  &        0.25                     &   -0.5                         &                             0.1 &        0.4                      &    0.1                       &2.99e-17     &     0.16                  &                       -0.10 &                    0.04   &                       0.66 &   1.91e-10  \\
                       & DeAm &                0.2484              &       0.5367                    &  1.10e-5   &        0.2199                     &  -0.5513                          &                             0.0885 &    0.1618                          &  0.1                         &    5.76e-9 &  0.15  & -0.11  & 0.03  & 0.74  & 2.22e-8     \\
\hline
\multirow{3}{*}{$p_3$} & true & \multicolumn{1}{c}{0.35}         & \multicolumn{1}{c}{0.7}      &  -   &0.4&-0.5&0.15&0.6&0.15& --    & 0.20  & -0.10  & 0.10  & 3  & -    \\
                       & Am   &           0.3476                   &      0.6984                     &  1.00e-4   &   0.4                          &  -0.5                          &0.15                              &      0.6                        &       0.15                    &7.03e-18     &         0.22              &                       -0.19 &                 0.07      &                       1.32 &   5.47e-10  \\
                       & DeAm &            0.3141                  &      0.5527                     &  5.99e-4   &                            0.3970 & -0.4892                           &         0.1517                     &                             0.5413 &         0.1494                  &  4.68e-9   &   0.19     &   -0.17  &  0.09  &  1.88 &   3.33e-7  \\
\hline
\multirow{3}{*}{$p_4$} & true & \multicolumn{1}{c}{0.425}         & \multicolumn{1}{c}{0.8}      &   -  &0.55&-0.45&0.2&1.2&0.2&--     & 0.10  & -0.10  & 0.20  & 5  &  -   \\
                       & Am   &            0.4262                  &          0.7966                 &  3.27e-6   &    0.55                         &  -0.45                          &0.2                              &         1.2                     &   0.2                        & 8.41e-22    &    0.10                   &                       -0.10 &                   0.20    &                       5.00 &    6.29e-16 \\
                       & DeAm &             0.3801                 &         0.6009                  &   1.96e-5  &   0.5625                          &    -0.4369                        &                             0.2035 &        1.2198                      & 0.1988                          &  4.50e-9   &     0.15  & -0.14  &  0.22 &   3.63   & 6.53e-7     \\
\hline
\multirow{3}{*}{$p_5$} & true & \multicolumn{1}{c}{0.5}         & \multicolumn{1}{c}{0.9}      &  -   &0.7&-0.8&0.3&1.4&0.3&  --   &  0.10  & -0.15  & 0.20  &  7 &  -   \\
                       & Am   &              0.4986                &    0.9036                       &   4.02e-6  & 0.7                            &   -0.8                         & 0.3                             &      1.4                        &    0.3                       & 8.58e-23    &          0.10             &                       -0.15 &              0.20         &                       7.00 &   5.00e-13  \\
                       & DeAm &                0.4430              &      0.6549                     &  2.38e-5   &      0.7763                       &  -0.7602                          &                             0.3073 &                1.7021              &                   0.2979        &  2.34e-8   &           0.05  &            -0.20  &   0.23  &    5.08 &    1.67e-6
\end{tabular}
\caption{Calibration results for calibrating to out-of-the-money put and call options combined. In any model, no option price violated condition~\eqref{cond:DisregardAtCalib}.}
\label{Tab_Calibration_Synthetic_Data_oom}
\end{sidewaystable}

==> tex/table_calibration_put.tex <==
\begin{sidewaystable}[]
\centering
\small
\begin{tabular}{cl|lll|llllll|lllll}
                       &      & \multicolumn{3}{c|}{CEV}                                       & \multicolumn{6}{c|}{Heston}                                                                                                                              & \multicolumn{5}{c}{Merton}                                                                          \\
                       &      & \multicolumn{1}{c}{$\sigma$} & \multicolumn{1}{c}{$\xi$} & aase & \multicolumn{1}{c}{$\zeta$} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{$\gamma$} & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{$v_0$} & aase & \multicolumn{1}{c}{$\sigma$} & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{$\beta$} & \multicolumn{1}{c}{$\lambda$} & aase \\
\hline
\multirow{3}{*}{$p_1$} & true & \multicolumn{1}{c}{0.2}         & \multicolumn{1}{c}{0.5}      &  -   & 0.1& -0.2&0.07 & 0.1& 0.07& --   & 0.20  & -0.01  & 0.01  & 1  &  -   \\
                       & Am   &                    0.1977          &        0.4962                   & 7.74e-6    &0.1002&   -0.1999&    0.07&0.1026&0.07&  1.43e-13   & 0.20  & 0.01  & 0.05  &   0.29    & 1.07e-10 \\
                       & DeAm &                     0.1894         &       0.4501                    &   8.35e-5  &  0.1&-0.4839&0.0651&0.5144&0.0695&1.50e-7     &  0.20  &      -0.06       & 0.03 &  0.37 & 8.37e-8 \\
\hline
\multirow{3}{*}{$p_2$} & true & \multicolumn{1}{c}{0.275}         & \multicolumn{1}{c}{0.6}      &    - & 0.25&-0.5&0.1&0.4&0.1& --    & 0.15  & -0.05  & 0.05  & 2  &   -  \\
                       & Am   &                 0.2740             &     0.6004                      &  4.98e-7   &0.25 &-0.5&0.1&0.4&0.1&6.47e-23& 0.15  &    -0.06    & 0.05    &  1.55  &  2.69e-11\\
                       & DeAm &                  0.2607            &     0.7539                      &  2.04e-6   & 0.2667&-0.5067&0.0978&0.4374&0.0992&3.28e-8     &  0.14  &  -0.10  & 0.01  &  1.31  &  1.63e-7 \\
\hline
\multirow{3}{*}{$p_3$} & true & \multicolumn{1}{c}{0.35}         & \multicolumn{1}{c}{0.7}      &  -   &0.4&-0.5&0.15&0.6&0.15& --    & 0.20  & -0.10  & 0.10  & 3  & -    \\
                       & Am   &              0.3515                &  0.7576                         &   4.37e-5  & 0.4&-0.5&0.15&0.6&0.15&7.15e-16     &   0.22   &     -0.19   &  0.07  &   1.31   & 8.83e-10\\
                       & DeAm &                0.3272              &        0.8528                  &   1.92e-4  &0.4684&-0.437&0.1544&0.6806&0.1495&6.04e-9  & 0.16  &   -0.05  &  0.11 & 5.04    & 3.12e-8 \\
\hline
\multirow{3}{*}{$p_4$} & true & \multicolumn{1}{c}{0.425}         & \multicolumn{1}{c}{0.8}      &  -   &0.55&-0.45&0.2&1.2&0.2&--     & 0.10  & -0.10  & 0.20  & 5  &  -   \\
                       & Am   &             0.4258                 &     0.7898                      &  1.53e-6   & 0.55&-0.45&0.2&1.2&0.2&1.44e-17     &   0.10   &   -0.10 & 0.20   &   5.00 &  1.22e-13\\
                       & DeAm &                  0.3942            &         0.8755                  &   7.30e-6  &0.5773&-0.4298&0.2046&1.1975&0.1986&2.86e-9     &   0.09   &   -0.09   &  0.21  &    4.90   &  2.19e-7 \\
\hline
\multirow{3}{*}{$p_5$} & true & \multicolumn{1}{c}{0.5}         & \multicolumn{1}{c}{0.9}      &   -  &0.7&-0.8&0.3&1.4&0.3&  --   &  0.10  & -0.15  & 0.20  &  7 &  -   \\
                       & Am   &                  0.4982            &     0.9036                      &  1.53e-6   &0.7&-0.8&0.3&1.4&0.3&1.68e-17     &   0.10    &  -0.15  &  0.20 &   7.00  &  8.96e-13 \\
                       & DeAm &                     0.4570         &        0.9192                   &   1.02e-5  &0.8504&-0.7057&0.3136&1.5832&0.2993&1.31e-8     &  0.05 & -0.11  &  0.21  &  7.95  & 1.73e-7
                       
\end{tabular}
\caption{Calibration results for calibrating to put options. Due to the effect of non-unique De-Americanization results, some option prices have been neglected in the calibration to De-Americanized option data, as Remark~\ref{rem:PutOptionsOutinCalib} explains. In scenarios $p_1$ to $p_5$ of the CEV model x, for the Heston model none and in scenario $p_1$ and $p_2$ of the Merton model, 5 prices have been excluded.}
\label{Tab_Calibration_Synthetic_Data_Put}
\end{sidewaystable}

==> tex/table_pricing_heston_backup.tex <==
%\begin{sidewaystable}[]\tiny
%\centering
%\setlength{\tabcolsep}{1mm}
%\begin{tabular}{cc|rrrrrrrr|rrrrrrrr|rrrrrrrr}
%&&\multicolumn{8}{c|}{Average Difference}&\multicolumn{8}{c|}{Maximal absolute difference}&\multicolumn{8}{c}{Maximal European price}\\
%&&$T_1$&$T_2$&$T_3$&$T_4$&$T_5$&$T_6$&$T_7$&$T_8$&$T_1$&$T_2$&$T_3$&$T_4$&$T_5$&$T_6$&$T_7$&$T_8$&$T_1$&$T_2$&$T_3$&$T_4$&$T_5$&$T_6$&$T_7$&$T_8$\\
%\hline	
%\multirow{5}{*}{$p_1$}&		$r=0\%$	&1.E-8	&	2.E-7	&	2.E-7	&	1.E-7	&	2.E-7	&	1.E-7	&	3.E-7	&	-3.E-7	&	1.E-6	&	8.E-7	&	7.E-7	&	2.E-7	&	7.E-7	&	6.E-7	&	2.E-6	&	2.E-6	&	0.200	&	0.202	&	0.205	&	0.209	&	0.217	&	0.229	&	0.240	&	0.278	\\
%&	$r=1\%$	&-7.E-5	&	-4.E-5	&	-5.E-5	&	-4.E-5	&	-4.E-5	&	-3.E-5	&	-3.E-5	&	6.E-6	&	3.E-4	&	1.E-4	&	1.E-4	&	9.E-5	&	7.E-5	&	6.E-5	&	5.E-5	&	6.E-5	&	0.199	&	0.200	&	0.202	&	0.205	&	0.212	&	0.222	&	0.231	&	0.261	\\
%&	$r=2\%$	&-9.E-5	&	-7.E-5	&	-9.E-5	&	-6.E-5	&	-5.E-5	&	-5.E-5	&	-4.E-5	&	3.E-5	&	3.E-4	&	1.E-4	&	2.E-4	&	1.E-4	&	1.E-4	&	8.E-5	&	5.E-5	&	1.E-4	&	0.198	&	0.198	&	0.200	&	0.202	&	0.207	&	0.214	&	0.221	&	0.244	\\
%&	$r=5\%$	&-3.E-4	&	-4.E-4	&	-1.E-4	&	-9.E-5	&	-9.E-5	&	-8.E-5	&	-7.E-5	&	3.E-5	&	5.E-4	&	2.E-3	&	2.E-4	&	1.E-4	&	2.E-4	&	2.E-4	&	9.E-5	&	3.E-4	&	0.195	&	0.193	&	0.191	&	0.191	&	0.192	&	0.194	&	0.195	&	0.198	\\
%&	$r=7\%$	&-3.E-4	&	-3.E-4	&	-9.E-4	&	-1.E-4	&	-8.E-5	&	-1.E-4	&	-1.E-4	&	-4.E-5	&	6.E-4	&	3.E-3	&	7.E-3	&	3.E-5	&	8.E-5	&	3.E-4	&	2.E-4	&	2.E-4	&	0.194	&	0.189	&	0.186	&	0.184	&	0.182	&	0.180	&	0.179	&	0.171	\\
%\hline	
%\multirow{5}{*}{$p_2$}&	$r=0\%$		&3.E-8	&	1.E-7	&	1.E-8	&	-2.E-7	&	3.E-7	&	4.E-7	&	-8.E-8	&	-3.E-8	&	5.E-7	&	5.E-7	&	4.E-7	&	5.E-7	&	7.E-7	&	7.E-7	&	1.E-6	&	2.E-7	&	0.201	&	0.204	&	0.208	&	0.214	&	0.224	&	0.238	&	0.251	&	0.293	\\
%&	$r=1\%$&-4.E-5	&	-3.E-5	&	-4.E-5	&	-3.E-5	&	-2.E-5	&	-1.E-5	&	-2.E-6	&	9.E-5	&	1.E-4	&	7.E-5	&	8.E-5	&	5.E-5	&	2.E-5	&	1.E-5	&	5.E-5	&	2.E-4	&	0.200	&	0.202	&	0.206	&	0.210	&	0.219	&	0.231	&	0.242	&	0.277	\\
%&	$r=2\%$&-1.E-4	&	-5.E-5	&	-6.E-5	&	-5.E-5	&	-4.E-5	&	-3.E-5	&	-8.E-6	&	1.E-4	&	7.E-4	&	1.E-4	&	1.E-4	&	6.E-5	&	2.E-5	&	3.E-5	&	9.E-5	&	4.E-4	&	0.199	&	0.200	&	0.203	&	0.207	&	0.214	&	0.224	&	0.233	&	0.261	\\
%&	$r=5\%$&-2.E-4	&	-7.E-5	&	-1.E-4	&	-9.E-5	&	-8.E-5	&	-9.E-5	&	-1.E-4	&	2.E-5	&	8.E-4	&	6.E-5	&	3.E-4	&	9.E-5	&	2.E-5	&	2.E-5	&	7.E-5	&	4.E-4	&	0.196	&	0.195	&	0.195	&	0.197	&	0.200	&	0.204	&	0.208	&	0.217	\\
%&	$r=7\%$&-2.E-4	&	-6.E-4	&	-1.E-4	&	-1.E-4	&	-1.E-4	&	-2.E-4	&	-2.E-4	&	-3.E-4	&	1.E-3	&	5.E-3	&	3.E-6	&	1.E-4	&	4.E-5	&	6.E-5	&	7.E-5	&	5.E-5	&	0.194	&	0.191	&	0.190	&	0.190	&	0.191	&	0.192	&	0.193	&	0.192	\\
%\hline	
%\multirow{5}{*}{$p_3$}&	$r=0\%$	&3.E-9	&	4.E-8	&	-3.E-7	&	3.E-9	&	8.E-8	&	-2.E-7	&	5.E-7	&	1.E-7	&	1.E-6	&	2.E-6	&	1.E-6	&	7.E-7	&	6.E-7	&	6.E-7	&	5.E-7	&	3.E-6	&	0.202	&	0.208	&	0.216	&	0.224	&	0.238	&	0.256	&	0.273	&	0.326	\\
%&	$r=1\%$&-3.E-5	&	-2.E-5	&	-3.E-5	&	-2.E-5	&	-6.E-6	&	1.E-5	&	3.E-5	&	2.E-4	&	8.E-5	&	5.E-5	&	4.E-5	&	1.E-5	&	2.E-5	&	6.E-5	&	1.E-4	&	3.E-4	&	0.201	&	0.207	&	0.213	&	0.220	&	0.233	&	0.250	&	0.264	&	0.309	\\
%&	$r=2\%$&-6.E-5	&	-4.E-5	&	-4.E-5	&	-3.E-5	&	-7.E-6	&	2.E-5	&	6.E-5	&	3.E-4	&	2.E-4	&	7.E-5	&	7.E-5	&	8.E-6	&	5.E-5	&	1.E-4	&	2.E-4	&	6.E-4	&	0.200	&	0.205	&	0.211	&	0.217	&	0.228	&	0.243	&	0.255	&	0.294	\\
%&	$r=5\%$&-1.E-4	&	-7.E-5	&	-9.E-5	&	-5.E-5	&	-2.E-5	&	2.E-5	&	7.E-5	&	5.E-4	&	2.E-4	&	1.E-4	&	1.E-4	&	1.E-5	&	1.E-4	&	3.E-4	&	4.E-4	&	1.E-3	&	0.197	&	0.199	&	0.203	&	0.207	&	0.215	&	0.224	&	0.231	&	0.250	\\
%&	$r=7\%$&-4.E-4	&	-9.E-5	&	-1.E-4	&	-7.E-5	&	-4.E-5	&	-2.E-5	&	1.E-5	&	4.E-4	&	2.E-3	&	1.E-4	&	2.E-4	&	2.E-5	&	2.E-4	&	3.E-4	&	4.E-4	&	8.E-4	&	0.195	&	0.196	&	0.198	&	0.201	&	0.206	&	0.212	&	0.216	&	0.225	\\
%\hline	
%\multirow{5}{*}{$p_4$}&	$r=0\%$	&2.E-8	&	-8.E-8	&	2.E-7	&	4.E-8	&	-5.E-7	&	-1.E-7	&	-4.E-7	&	2.E-7	&	4.E-8	&	8.E-7	&	2.E-6	&	4.E-8	&	2.E-6	&	2.E-6	&	3.E-6	&	2.E-6	&	0.204	&	0.214	&	0.224	&	0.234	&	0.252	&	0.275	&	0.295	&	0.362	\\
%&	$r=1\%$&-3.E-5	&	-2.E-5	&	-2.E-5	&	-1.E-5	&	2.E-6	&	2.E-5	&	5.E-5	&	2.E-4	&	7.E-5	&	3.E-5	&	2.E-5	&	2.E-6	&	3.E-5	&	6.E-5	&	9.E-5	&	3.E-4	&	0.203	&	0.212	&	0.221	&	0.231	&	0.247	&	0.268	&	0.287	&	0.345	\\
%&	$r=2\%$&-5.E-5	&	-3.E-5	&	-3.E-5	&	-1.E-5	&	1.E-5	&	5.E-5	&	9.E-5	&	4.E-4	&	1.E-4	&	4.E-5	&	4.E-5	&	2.E-5	&	7.E-5	&	1.E-4	&	2.E-4	&	6.E-4	&	0.202	&	0.210	&	0.219	&	0.227	&	0.243	&	0.262	&	0.278	&	0.329	\\
%&	$r=5\%$&-1.E-4	&	-5.E-5	&	-6.E-5	&	-1.E-5	&	4.E-5	&	1.E-4	&	2.E-4	&	8.E-4	&	3.E-4	&	6.E-5	&	7.E-5	&	8.E-5	&	2.E-4	&	3.E-4	&	4.E-4	&	1.E-3	&	0.199	&	0.205	&	0.211	&	0.218	&	0.229	&	0.243	&	0.255	&	0.286	\\
%&	$r=7\%$&-1.E-4	&	-6.E-5	&	-8.E-5	&	-1.E-5	&	4.E-5	&	1.E-4	&	2.E-4	&	9.E-4	&	3.E-4	&	6.E-5	&	9.E-5	&	1.E-4	&	3.E-4	&	4.E-4	&	5.E-4	&	1.E-3	&	0.197	&	0.202	&	0.207	&	0.212	&	0.221	&	0.231	&	0.240	&	0.259	\\
%\hline	
%\multirow{5}{*}{$p_5$}&	$r=0\%$	&-1.E-7	&	-3.E-7	&	-3.E-7	&	2.E-7	&	5.E-8	&	8.E-7	&	1.E-6	&	-2.E-6	&	5.E-7	&	4.E-7	&	2.E-7	&	4.E-7	&	8.E-7	&	4.E-6	&	6.E-6	&	4.E-6	&	0.207	&	0.222	&	0.234	&	0.248	&	0.270	&	0.297	&	0.322	&	0.400	\\
%&	$r=1\%$&-2.E-5	&	-2.E-5	&	-2.E-5	&	-7.E-6	&	2.E-5	&	8.E-5	&	2.E-4	&	7.E-4	&	6.E-5	&	3.E-5	&	2.E-5	&	9.E-6	&	6.E-5	&	2.E-4	&	3.E-4	&	1.E-3	&	0.206	&	0.220	&	0.232	&	0.245	&	0.265	&	0.291	&	0.314	&	0.384	\\
%&	$r=2\%$&-4.E-5	&	-3.E-5	&	-4.E-5	&	-1.E-5	&	3.E-5	&	1.E-4	&	3.E-4	&	1.E-3	&	1.E-4	&	5.E-5	&	5.E-5	&	1.E-5	&	1.E-4	&	3.E-4	&	5.E-4	&	2.E-3	&	0.205	&	0.218	&	0.230	&	0.242	&	0.261	&	0.285	&	0.306	&	0.369	\\
%&	$r=5\%$&-1.E-4	&	-7.E-5	&	-1.E-4	&	-5.E-5	&	2.E-5	&	2.E-4	&	5.E-4	&	2.E-3	&	2.E-4	&	1.E-4	&	1.E-4	&	3.E-5	&	1.E-4	&	4.E-4	&	9.E-4	&	3.E-3	&	0.202	&	0.213	&	0.223	&	0.233	&	0.249	&	0.268	&	0.283	&	0.326	\\
%&	$r=7\%$&-1.E-4	&	-1.E-4	&	-1.E-4	&	-9.E-5	&	-1.E-5	&	2.E-4	&	5.E-4	&	3.E-3	&	3.E-4	&	1.E-4	&	2.E-4	&	9.E-5	&	6.E-5	&	4.E-4	&	8.E-4	&	3.E-3	&	0.201	&	0.210	&	0.219	&	0.227	&	0.241	&	0.257	&	0.269	&	0.300	\\
%\hline	
%\end{tabular}
%\caption{Summary of De--Ameri\-cani\-za\-tion effects on pricing put options in the Heston model}
%\label{Tab_Pricing_Heston}
%\end{sidewaystable}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]\scriptsize
\centering
\begin{tabular}{lc|cccccccc}
\multicolumn{1}{c}{}                    &   & \multicolumn{8}{c}{Maximal absolute difference} \\
\multicolumn{1}{c}{}                    &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multicolumn{1}{c}{\multirow{5}{*}{p1}} & 0 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 1 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 2 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 5 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 7 &      &      &     &     &     &     &     &     \\
\hline
\multicolumn{1}{c}{}                    &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multicolumn{1}{c}{\multirow{5}{*}{p1}} & 0 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 1 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 2 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 5 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 7 &      &      &     &     &     &     &     &     \\
\hline
\multicolumn{1}{c}{}                    &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multicolumn{1}{c}{\multirow{5}{*}{p1}} & 0 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 1 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 2 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 5 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 7 &      &      &     &     &     &     &     &     \\
\hline
\multicolumn{1}{c}{}                    &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multicolumn{1}{c}{\multirow{5}{*}{p1}} & 0 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 1 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 2 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 5 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 7 &      &      &     &     &     &     &     &     \\
\hline
\multicolumn{1}{c}{}                    &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multicolumn{1}{c}{\multirow{5}{*}{p1}} & 0 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 1 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 2 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 5 &      &      &     &     &     &     &     &     \\
\multicolumn{1}{c}{}                    & 7 &      &      &     &     &     &     &     &     \\
\hline
                                        &   & \multicolumn{8}{c}{Maximal European price}      \\
                                        &   & 1    & 2    & 3   & 4   & 5   & 6   & 7   & 8   \\ \hline
\multirow{5}{*}{p1}                     & 0 &      &      &     &     &     &     &     &     \\
                                        & 1 &      &      &     &     &     &     &     &     \\
                                        & 2 &      &      &     &     &     &     &     &     \\
                                        & 5 &      &      &     &     &     &     &     &     \\
                                        & 7 &      &      &     &     &     &     &     &   \\
 \hline
\multirow{5}{*}{p1}                     & 0 &      &      &     &     &     &     &     &     \\
                                        & 1 &      &      &     &     &     &     &     &     \\
                                        & 2 &      &      &     &     &     &     &     &     \\
                                        & 5 &      &      &     &     &     &     &     &     \\
                                        & 7 &      &      &     &     &     &     &     &   \\
 \hline
\multirow{5}{*}{p1}                     & 0 &      &      &     &     &     &     &     &     \\
                                        & 1 &      &      &     &     &     &     &     &     \\
                                        & 2 &      &      &     &     &     &     &     &     \\
                                        & 5 &      &      &     &     &     &     &     &     \\
                                        & 7 &      &      &     &     &     &     &     &\\   
  \hline
\multirow{5}{*}{p1}                     & 0 &      &      &     &     &     &     &     &     \\
                                        & 1 &      &      &     &     &     &     &     &     \\
                                        & 2 &      &      &     &     &     &     &     &     \\
                                        & 5 &      &      &     &     &     &     &     &     \\
                                        & 7 &      &      &     &     &     &     &     &\\                                          
                                                                                  \hline
\multirow{5}{*}{p1}                     & 0 &      &      &     &     &     &     &     &     \\
                                        & 1 &      &      &     &     &     &     &     &     \\
                                        & 2 &      &      &     &     &     &     &     &     \\
                                        & 5 &      &      &     &     &     &     &     &     \\
                                        & 7 &      &      &     &     &     &     &     &   
\end{tabular}
\caption{Summary of De--Ameri\-cani\-za\-tion effects on pricing put options in the Heston model}
\label{Tab_Pricing_Heston}
\end{table}

==> tex/titlepage.tex <==
\thispagestyle{empty}
	\begin{center}
	{\bfseries\Large Calibration by De--Americanization}
		\par\bigskip
		\vspace{1cm}
		
%	{\Large Maximilian Ga\ss}\\
%		\vspace{0.2cm}
%		{Chair of Mathematical Finance,}\\ 
%		{Technische Universit{\"a}t M{\"u}nchen,}\\
%		{Parkring 11, 85748 Garching-Hochbr\"uck, Germany,}\\
%		{email: maximilian.gass@tum.de,}\\
%		{phone: +49 89 289 18790.}\\
%		\vspace{1cm}
%		
%	{\Large Kathrin Glau}\\
%		\vspace{0.2cm}
%		{Chair of Mathematical Finance,}\\ 
%		{Technische Universit{\"a}t M{\"u}nchen,}\\
%		{Parkring 11, 85748 Garching-Hochbr\"uck, Germany,}\\
%		{email: kathrin.glau@tum.de,}\\
%		{phone: +49 89 289 17403.}\\
	\end{center}
\vspace{3cm}


\begin{abstract}
We investigate a market practitioner's approach to calibration called De--Ameri\-cani\-za\-tion. Instead of calibrating market models to American option prices directly, these are de-americanized first by calibrating a simple tree model and then using the calibrated tree model to generate respective European option prices.  More sophisticated models can then be calibrated to these pseudo-European option prices. The effect of this approximation is tested for a variety of models including the Heston and L\'evy driven models. Being able to calibrate these to American option prices directly, we conduct comparisons to the De-Americanization approach. Both, scenarios where the practitioner's approximation makes sense as well as cases where the routine generates unsatisfactory results are described.
	\end{abstract}
\minisec{Keywords}
	American options, calibration, binomial tree model, Heston model, L\'evy models, finite element methods


==> tex/tree.tex <==
\section{De--Ameri\-cani\-za\-tion: The Binomial Tree}
In this section we briefly introduce the binomial tree which is used to translate American option prices into European option prices. The binomial model was introduced by \cite{crr_tree}. An illustrative example is given in Figure \ref{tree}.%\todo{Figure anpassen} 
Basically, the tree approach models asset movements as follows. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.5\textwidth]{./fig/Multi-Step-Binomial-Model.png}
\caption{Scheme of the binomial tree}
\label{tree}
\end{center}
\end{figure}
Starting with an underlying value $S_0$ and a maturity $T$, the process $S_t$ is described over $n$ discrete time steps $\frac{T}{n}$. In each step of the tree the underlying moves up by factor $u$ or down by $d=\frac{1}{u}$. 


Once, the underlying values are derived in the tree, options can be valuated. Starting at each final node, the option value is the exercise value. Then, the option value is determined at each node in the binomial tree working backwards from the second last time step to the first node of the tree.  At each node, the option value is derived via risk-neutral valuation. At each node the probability of an upward resp. downward movement is given by $p=\frac{e^{\frac{rT}{n}}-\frac{1}{u}}{u-\frac{1}{u}}$ (up) resp. by $1-p$ (down). Then the option value at the first note is the option value at the valuation date. Applying this scheme will result in the option price for an European option. For American options at each node in the tree the option value derived via risk-neutral valuation is compared to the exercise value and the greater value is taken as option value at this node.\\ 
In our case, the tree is used to translate American option prices into European option prices: Given an American option, we know strike, maturity, price and interest rate. Thus, by looking at the tree, only the value for $u$ is unknown and can be derived such that the tree price matches the observed option price. Then, exactly this $u$ value is used to price the according European option with same maturity and strike. In Figure \ref{Toy_Example} a binomial tree as well as valuation of European and American options is illustrated.\\
In this way, every American option price is translated in an European option price individually. 
\begin{remark}
\cite{crr_tree} suggest $u=e^{\sigma\sqrt{t}}$. Thus, implicitly by applying the binomial tree to translate American prices into European prices by determining the according $u$ value for each option individually, the corresponding implicit $\sigma$ value is found.
\end{remark}
